Riemannian Langevin Algorithm for Solving Semidefinite Programs

We propose a Langevin diffusion-based algorithm for non-convex optimization and sampling on a product manifold of spheres. Under a logarithmic Sobolev inequality, we establish a guarantee for finite iteration convergence to the Gibbs distribution in terms of Kullback--Leibler divergence. We show that with an appropriate temperature choice, the suboptimality gap to the global minimum is guaranteed to be arbitrarily small with high probability. As an application, we consider the Burer--Monteiro approach for solving a semidefinite program (SDP) with diagonal constraints, and analyze the proposed Langevin algorithm for optimizing the non-convex objective. In particular, we establish a logarithmic Sobolev inequality for the Burer--Monteiro problem when there are no spurious local minima, but under the presence saddle points. Combining the results, we then provide a global optimality guarantee for the SDP and the Max-Cut problem. More precisely, we show that the Langevin algorithm achieves $\epsilon$ accuracy with high probability in $\widetilde{\Omega}( \epsilon^{-5} )$ iterations.

==> app_comparison.tex <==


\section{Discussion on \cite{wang2020fast}}
\label{sec:app_comparison}

In this section, 
we discuss an issue found in the proof of 
\cite[Lemma C.3]{wang2020fast}.

To start, we recall the authors are working with 
a general $d$-dimensional compact Riemannian manifold $(M,g)$, 
and let us assume the potential $F=0$ for simplicity. 
The proposed Langevin algorithm based on exponential maps  
\citep[Equation (1)]{wang2020fast} 
can be stated in Riemannian normal coordinates 
as a continuous time process for a single step 
\citep[Lemma C.3]{wang2020fast} 
\begin{equation}
	Y_t 
		= \exp\left( Y_0, \sqrt{2 t} \xi \right) \,, 
\end{equation}
where $\xi \sim N(0, I_d)$ is understood 
in normal coordinates of the tangent space at $T_{Y_0} M$. 
And the authors proceeds to write an SDE representation 
in normal coordinates centered at $Y_0$ 
\begin{equation}
\label{eq:flat_bm}
	dY_t = \sqrt{2} \, dB_t \,, 
\end{equation}
where $\{B_t\}_{t\geq 0}$ is 
a standard Brownian motion in $\mathbb{R}^d$, 
and this SDE holds up until $Y_t$ exits the normal neighbourhood. 

We summarize the main issue in the next proposition. 

\begin{proposition}

Let $\rho_t$ be the density of $Y_t$ on $M$. 
Then in general, $\rho_t$ \textbf{does not satisfy} 
the following Fokker--Planck equation 
\begin{equation}
\label{eq:bm_fpe}
	\de_t \rho_t = \Delta \rho_t \,, 
\end{equation}
where $\Delta$ is the Laplace--Beltrami operator. 

\end{proposition}

\begin{proof}

The core issue is that $\{Y_t\}_{t\geq 0}$ defined by \cref{eq:flat_bm} 
is not a Brownian motion on $M$ (adjusted for $\sqrt{2}$ time). 
Recalling \cite[Example 3.3.5]{hsu2002stochastic}, 
a Brownian motion $\{W_t\}_{t \geq 0}$ on $M$ 
(adjusted for $\sqrt{2}$ time) 
has the following SDE 
\begin{equation}
	dW_t^i = \sqrt{2} \sigma^i_j(W_t) \, dB_t^j 
		- g^{\ell k}(W_t) \Gamma^i_{k\ell} (W_t) \, dt \,, 
\end{equation}
where $\sigma$ is the positive definite square root of the matrix $g^{-1}$, 
$g^{\ell k}$ is the inverse Riemannian metric in normal coordinates, 
and $\Gamma^i_{k\ell}$ is the Christoffel symbol. 
Therefore $\{Y_t\}_{t\geq 0}$ cannot be a Brownian motion on $M$. 

At the same time, the only diffusion process on $M$ corresponding 
to this Fokker--Planck equation is 
the Brownian motion on manifold $\{W_t\}_{t\geq 0}$ 
\citep[Proposition 3.2.1]{hsu2002stochastic}. 
Therefore $\rho_t$ does not satisfy the Fokker--Planck equation 
\cref{eq:bm_fpe}. 

\end{proof}

The rest of the proof of \cite[Lemma C.3]{wang2020fast} 
depends on this key step, 
and therefore the consequences do not follow. 
In fact, we can compute the generator of $\{Y_t\}_{t\geq 0}$ 
as the ``flat Laplacian'' in normal coordinates 
\begin{equation}
	\lim_{t\to 0} \frac{1}{t} \mathbb{E}[ \phi(Y_t) - \phi(Y_0) | Y_0 = x ] 
	= 
	\sum_{i=1}^d \de_{i} \de_i \phi \,, 
	\quad 
	\forall \phi \in C^2(M) \,, 
\end{equation}
which we contrast with the Laplace--Beltrami operator 
in coordinates as 
\begin{equation}
	\Delta \phi 
	= 
		\frac{1}{\sqrt{ \det g }} \de_j \left( 
			\sqrt{\det g} g^{ij} \de_i \phi 
		\right) 
	= 
		g^{ij} \de_i \de_j \phi 
		+ g^{jk} \Gamma^i_{jk} \de_i \phi \,. 
\end{equation}




































































==> app_lyapunov.tex <==



==> app_normal.tex <==



==> app_revision.tex <==

\section{Revision Lemmas Needed}





\begin{lemma}[Smooth Partition Function]
\label{lm:smooth_partition}
For all $r_2 > r_1 > 0$ and $\epsilon > 0$, 
there exists a smooth non-increasing function 
$\psi : \mathbb{R} \to [0,1]$ such that 
\begin{equation}
	\psi(x) 
	= 
	\begin{cases}
		0 \,, & x \leq r_1 \,, \\ 
		\text{Decreasing} \,, & x \in (r_1, r_2) \,, \\ 
		1 \,, & x \geq r_2 \,, 
	\end{cases}
\end{equation}
and that $\| \psi^\prime \|_\infty \leq \frac{1}{r_2 - r_1} + \epsilon$. 
\end{lemma}

\begin{proof}

We start by defining the unit smooth bump function 
\begin{equation}
	\phi_b(x) 
	= 
	\begin{cases}
		\frac{ \exp\left( \frac{-1}{b^2 - x^2} \right) }{ 
				\int_{-b}^b \exp\left( \frac{-1}{b^2 - y^2} \right) \, dy 
				} 
				\,, & x \in [-b,b] \,, \\ 
		0 \,, & \text{ otherwise.}
	\end{cases}
\end{equation}

Observe that as $b\to 0$, $\phi_b$ converges to 
the Dirac delta functional with unit mass. 
This allows us to construct the derivative of $\psi$ as follows 
\begin{equation}
\begin{aligned}
	\psi^\prime(x) 
	&= 
		\left( \frac{1}{r_2 - r_1} + \epsilon \right) 
		\int_{-\infty}^x \phi_b(y - r_1 - b) - \phi_b(y - r_2 + b) \, dy 
		\\ 
	&= 
	\begin{cases}
		0 \,, & x \leq r_1 \text{ or } x \geq r_2 \,, \\ 
		\frac{1}{r_2 - r_1} + \epsilon \,, & x \in (r_1 + 2b, r_2 - 2b) \,, 
	\end{cases}
\end{aligned}
\end{equation}
where without loss of generality we can assume $b>0$ 
is sufficiently small for $\psi^\prime$ to be well defined. 

Then we can construct $\psi$ as 
\begin{equation}
	\psi(x) = \int_{-\infty}^x \psi^\prime(y) \, dy \,. 
\end{equation}

Finally, to satisfy the requirement that $\psi$ 
choose $b>0$ sufficiently small such that $\psi(r_2) = 0$, 
or more precisely 
\begin{equation}
	\int_{r_1}^{r_2} \psi^\prime(x) \, dx 
	= 
	\left( \frac{1}{r_2 - r_1} + \epsilon \right) 
	\int_{r_1}^{r_2} 
		\int_{-\infty}^x \phi_b(y - r_1 - b) - \phi_b(y - r_2 + b) \, dy  \, dx 
	= 1 \,. 
\end{equation}

Since this is always possible for $\epsilon$ small, 
therefore it's sufficient for the upper bound. 

\end{proof}


We first adapt one of the main results of \cite{cattiaux2013poincare} 
to extract an explicit Poincar\'e constant. 

\begin{proposition}[Adapted Theorem 2.3 of \cite{cattiaux2013poincare}]
\label{prop:poincare_adapted}
For all $r > \wt{r} > 0$, let us define 
the following open neighbourhoods of saddle points 
\begin{equation}
	B = \left\{ x \in M \, | \,  d_g(x, \mathcal{S}) < r \right\} \,, \quad 
	\wt B = \left\{ x \in M \, | \, d_g(x, \mathcal{S}) < \wt r \right\} \,. 
\end{equation}
Suppose $(\wt{B}^c, \nu|_{\wt{B}^c}, \Gamma|_{\wt{B}^c})$ 
satisfies a Poincar\'e inequality with constant $\kappa_{\wt{B}^c}$, 
and there exists $W \in C^2(B)$ such that $W \geq 1$ and 
\begin{equation}
	L W \leq - \theta W \,, \quad x \in B \,. 
\end{equation}
Then we have that $(M, \nu, \Gamma)$ satisfies a Poincar\'e inequality 
with constant 
\begin{equation}
	\frac{1}{\kappa} = \frac{4}{\theta} + 
		\left( \frac{4}{\theta \beta (r - \wt{r})^2 } + 2 \right) 
		\frac{1}{\kappa_{\wt{B}^c}} \,. 
\end{equation}
\end{proposition}

\begin{proof}

We will follow the steps of (H1) $\Rightarrow$ (H4) in \cite{cattiaux2013poincare} 
and first compute for any smooth $f$ and use integration-by-parts to write 
\begin{equation}
\begin{aligned}
	\int \frac{-LW}{W} f^2 \, d\nu 
	&= \int \Gamma\left( \frac{f^2}{W} , W \right) \, d\nu 
		\\ 
	&= 2 \int \frac{f}{W} \Gamma(f, W) \, d\nu 
		- \int \frac{f^2}{W^2} \Gamma(W, W) \, d\nu 
		\\ 
	&= - \int \left| \frac{f}{W \sqrt{\beta}} \grad W 
		- \frac{1}{\sqrt{\beta}} \grad f
		\right|^2 \, d\nu 
		+ 
		\int \Gamma(f,f) \, d\nu 
		\\ 
	&\leq \int \Gamma(f,f) \, d\nu \,. 
\end{aligned}
\end{equation}

Next we will introduce a partition function $\chi:M \to [0,1]$ 
such that $\chi = 1$ on $B^c$ and $\chi = 0$ on $\wt B$. 
This function can be explicitly constructed by choosing $\psi$ 
from \cref{lm:smooth_partition} with $r_1 = \wt{r}, r_2 = r$, and any $\epsilon>0$, 
then we can define 
\begin{equation}
	\chi(x) = \psi\left( d_g(x, \mathcal{S}) \right) \,, 
\end{equation}
where we recall $B, \wt{B}$ are neighbourhoods of $\mathcal{S}$. 
Here we note since $\|\psi^\prime\|_\infty \leq \frac{1}{r - \wt{r}} + \epsilon$, 
we also have that 
\begin{equation}
	\| \Gamma(\chi, \chi) \|_\infty 
	= \frac{1}{\beta} \| \psi^\prime \|_\infty^2 
	\leq \frac{1}{\beta} \left( \frac{1}{r - \wt{r}} + \epsilon \right)^2 \,. 
\end{equation}

This allows us to carry on the calculation with 
\begin{equation}
\begin{aligned}
	\int f^2 \, d\nu 
	&= \int (f(1-\chi) + f\chi)^2 \, d\nu \\ 
	&\leq 2 \int f^2 (1-\chi)^2 \, d\nu + 2 \int f^2 \chi^2 \, d\nu \\ 
	&\leq \frac{2}{\theta} \int \frac{-LW}{W} f^2 (1-\chi)^2 \, d\nu 
		+ 2 \int_{\wt B^c} f^2 \, d\nu \\ 
	&\leq \frac{2}{\theta} \int \Gamma( f(1-\chi), f(1-\chi) ) \, d\nu 
		+ 2 \int_{\wt B^c} f^2 \, d\nu \,. 
\end{aligned}
\end{equation}

Next we can use $\Gamma(fg, fg) \leq 2( f^2 \Gamma(g, g) + g^2 \Gamma(f,f) )$ 
to write 
\begin{equation}
\begin{aligned}
	\int f^2 \, d\nu 
	&\leq \frac{4}{\theta} \int \Gamma(f,f) \, d\nu 
		+ \frac{4}{\theta} \int f^2 \Gamma(\chi,\chi) \, d\nu 
		+ 2 \int_{\wt B^c} f^2 \, d\nu 
		\\ 
	&\leq \frac{4}{\theta} \int \Gamma(f,f) \, d\nu 
		+ \left( \frac{4 \|\Gamma(\chi, \chi)\|_\infty }{ \theta } + 2 \right) 
		\int_{\wt B^c} f^2 \, d\nu \,. 
\end{aligned}
\end{equation}

Since $(\wt B^c, \nu|_{\wt B^c}, \Gamma|_{\wt B^c})$ 
satisfies a Poincar\'e inequality, 
we have that for $\wt f = f - \int_{\wt B^c} f \, d\nu$ 
\begin{equation}
	\int_{\wt B^c} \wt f^2 \, d \nu 
	\leq 
	\frac{1}{ \kappa_{\wt B^c} } \int_{\wt B^c} \Gamma(f, f) \, d\nu \,, 
\end{equation}
which implies 
\begin{equation}
	\text{Var}_\nu(f) \leq \int \wt f^2 \, d\nu 
	\leq 
	\left( \frac{4}{\theta} 
	+ \left( \frac{4 \| \Gamma(\chi, \chi) \|_\infty }{ \theta } 
	\right) \kappa_{ \wt B^c } 
	\right) 
	\int \Gamma(f, f) \, d\nu \,. 
\end{equation}

Finally, we explicitly control the constant 
\begin{equation}
	\frac{4}{\theta} 
	+ \left( \frac{4 \| \Gamma(\chi, \chi) \|_\infty }{ \theta } 
	\right) \kappa_{ \wt B^c } 
	\leq 
	\frac{4}{\theta} 
	+ \left( \frac{4}{ \theta \beta } 
	\left( \frac{1}{r - \wt r} + \epsilon
	\right)^2 
	\right) \frac{1}{ \kappa_{\wt B^c} } \,, 
\end{equation}
and since $\psi$ can be constructed for any $\epsilon > 0$, 
we have the Poincar\'e constant  
\begin{equation}
	\frac{1}{\kappa} 
	= \frac{4}{\theta} 
	+ \left( \frac{4}{ \theta \beta (r - \wt r)^2 } 
	\right) \frac{1}{ \kappa_{\wt B^c} } \,. 
\end{equation}

\end{proof}









\begin{proposition}
[Poincar\'{e} Inequality on $M$]
\label{prop:lyapunov_poincare_adapted}
Suppose $F$ satisfies 
\cref{asm:app_c3,asm:app_morse,asm:app_unique_min} 
and $d \geq 2$. 
Then for all choices of $a,\beta > 0$ such that 
\begin{equation}
\begin{aligned}
	a^2 
	&\geq 
		\frac{6 K_2 nd}{ C_F^2 } 
		\,, \\ 
	\beta 
	&\geq
		a^2 
		\max\left( 
			\, \frac{ 4 K_3^2 }{ \lambda_{*}^2 } \,, 
			\, \frac{a^4}{4} (K_3 + 2K_2)^2 \, 
		 \right) \,, 
\end{aligned}
\end{equation}
where $\lambda_{*}$ is defined in \cref{asm:app_morse}, 
we have that the Markov triple $(M, \nu, \Gamma)$ 
satisfies a Poincar\'{e} inequality with constant 
\begin{equation}
	\kappa
	= 
		\frac{1}{(1 + \frac{1}{ 2\kappa_U } ) + (2 + \frac{16}{3 \lambda_*})}
	\geq 
		\begin{cases}
			\frac{\lambda_*^2}{14} \,, 
			& \text{ if the global minimum is unique, } \\
			\frac{\lambda_*}{11 \beta} \,, 
			& \text{ otherwise. } 
		\end{cases}
		\,, 
\end{equation} 
where $\kappa_U$ is the Poincar\'{e} constant 
from \cref{lm:poincare_near_min}. 

\end{proposition}

\begin{proof}

Using \cref{lm:lyapunov_poincare_ua}, 
we know that $\nu$ restricted to $U \cup A$ 
already satisfies a Poincar\'{e} inequality with constant 
$\kappa_{U \cup A}$, 
therefore it is sufficient to establish a Lyapunov condition 
on $B = M \ (U \cup A)$. 

To this goal, we will use the escape time definition. 
More precisely, we will define the escape time 
\begin{equation}
	\tau_{B^c} := \left\{ t \geq 0 | Z_t \notin B \right\} \,, 
\end{equation}
and define the Lyapunov function as 
\begin{equation}
	W_2(x) := \mathbb{E} [ e^{ \wt{\lambda} \tau_{B^c} / 4 } | Z_0 = x ] \,. 
\end{equation}


Using the equivalent characterization of sub-exponential 
random variables \cref{thm:subexp_equiv_wainwright} 
and the escape time bound \cref{prop:local_escape_time_bound} 
with the condition on $\beta$, 
we get that 
\begin{equation}
	\mathbb{E} [ e^{ \lambda_* \tau_{B^c} / 4 } | Z_0 = x ] < \infty \,, 
	\quad \text{ for all } \, x \in B \,. 
\end{equation}

Then we can use \cref{cor:escape_time_lyapunov} 
to establish the Lyapunov condition 
\begin{equation}
	\frac{L W_2}{W_2} 
	\leq 
		- \frac{\lambda_*}{4} \,, 
		\quad 
	x \in B \,. 
\end{equation}

At this point we can once again use 
\cref{prop:poincare_adapted} 
with $\theta = \lambda_* / 4$ 
and $\kappa_{\wt B^c}$ from \cref{lm:lyapunov_poincare_ua} 
for $\wt r = \frac{a}{2 \sqrt{\beta}}, r = 2 \wt r$, 
which implies that $(M, \nu, \Gamma)$ satisfies 
a Poincar\'{e} inequality with constant 
\begin{equation}
	\frac{1}{ \kappa }
	= 
		\frac{16}{\lambda_*} + 
		\left( \frac{16}{\lambda_* \beta} \frac{4 \beta}{a^2} \right) 
		\left( 1 + \frac{1}{2\kappa_U} \right) 
		\,. 
\end{equation}

Using simplifying bounds with $C_F \leq 1, K_2 \geq 1, d \geq 2, n \geq 1$, 
we can write $\frac{1}{a^2} \leq \frac{C_F^2}{6K_2 nd} \leq \frac{1}{12}$, 
and therefore get 
\begin{equation}
	\frac{1}{ \kappa }
	\leq 
		\left( 1 + \frac{1}{2 \kappa_U} \right) 
		\left( \frac{16}{3 \lambda_*} + 2 \right) \,, 
\end{equation}
as desired. 

We will further simplify this result by the two cases of $\kappa_U$. 
Firstly when the global minimum is unique 
and therefore $\kappa_U = \frac{1}{2} \lambda_*$, 
we can use the simplifying bound of $\lambda_* \leq 1$ to write 
\begin{equation}
	\frac{1}{\kappa}
	= 
		\left(1 + \frac{1}{\lambda_*}\right) 
		\left(2 + \frac{16}{3 \lambda_*} \right) 
	\leq 
		\frac{\lambda_*^2}{14} \,. 
\end{equation}

At the same time, when $\kappa_U = \frac{d-1}{\beta}$, 
we use the fact that $d \geq 2, \lambda_* \leq 1, \beta \geq 1$ 
to get a bound 
\begin{equation}
	\frac{1}{\kappa}
	= 
		\left( 1 + \frac{\beta}{2(d-1)} \right) 
		\left( 2 + \frac{16}{3 \lambda_*} \right) 
	\leq 
		\frac{11 \beta}{\lambda_*} \,. 
\end{equation}

Putting these bounds together gives us the desired result. 

\end{proof}


































\begin{proposition}
[Poincar\'e Implies LSI]
\label{prop:poincare_implies_lsi}
Suppose that $(M,g)$ is the product of $n$ unit spheres $S^d$, 
with $F \in C^2(M)$, 
and $\nu = \frac{1}{Z} \exp( -\beta F )$ with $\beta \geq 1$. 
Suppose further that 
\begin{enumerate}
	\item There exists a constant $K > 0$ such that 
		\begin{equation}
			\nabla^2 F + \frac{1}{\beta} \Ric_g 
			\geq - K g \,, 
		\end{equation}
	\item $(M, \nu, \Gamma)$ satisfies a Poincar\'{e} 
		inequality with constant $1 \geq \kappa > 0$. 
\end{enumerate}
Then we have that $(M, \nu, \Gamma)$ satisfies 
a logarithmic Sobolev inequality with constant 
\begin{equation}
	\frac{1}{\alpha} 
	= \frac{11 \beta K n }{\kappa} \,. 
\end{equation}
\end{proposition}

\begin{proof}

We start by defining the ``unadjusted'' Fisher information as 
$\wt I_\nu(\mu) = \beta I_\mu(\mu) = \int |\grad h|^2 / h \, d\nu$, 
where $h = \frac{d\mu}{d\nu}$.  
Then we can apply the HWI inequality 
from \cref{thm:hwi_inequality} 
to $V = \beta F$, 
which gives us 
\begin{equation}
	H_\nu( \mu ) 
	\leq 
		W_2( \mu, \nu ) \sqrt{ \wt I_\nu(\mu) } 
		+ \frac{\beta K}{2} 
			W_2^2(\mu, \nu) \,. 
\end{equation}

Now using the trivial bound 
$W_2(\mu,\nu)^2 \leq \sup_{x,y} d_g(x,y)^2 \leq \pi^2 n$ 
and Young's inequality with 
$ab \leq \frac{\tau}{2} a^2 + \frac{1}{2 \tau} b^2$, 
we can write 
\begin{equation}
\begin{aligned}
	H_\nu( \mu ) 
	&\leq 
		\frac{\tau}{2} \wt I_\nu(\mu) 
		+ \left( \frac{1}{2\tau} + \frac{\beta K}{2} \right) 
			W_2^2(\mu, \nu) 
			\\ 
	&\leq 
		\frac{\tau}{2} \wt I_\nu(\mu) 
		+ \left( \frac{1}{2\tau} + \frac{\beta K}{2} \right) 
		\pi^2 n 
		\\ 
	&\leq 
		\frac{\tau \beta}{2} \wt I_\nu(\mu) 
		+ \left( \frac{1}{2\tau} + \frac{\beta K}{2} \right) 
		\pi^2 n 
		\\ 
	&=: 
		A I_\nu(\mu) + B \,, 
\end{aligned}
\end{equation}
which is a defective logarithmic Sobolev inequality. 

Using a standard tightening argument 
with a Poincar\'{e} inequality via Rothaus' Lemma 
\citep[Proposition 5.1.3]{bakry2013analysis}, 
we have that a tight logarithmic Sobolev inequality 
\begin{equation}
\begin{aligned}
	H_\nu( \mu ) 
	&\leq 
		\left[ A + \frac{B+2}{\kappa} \right] 
		\, I_\nu(\mu) \\ 
	&= 
		\left( \frac{\tau \beta}{2} 
			+ \frac{ \frac{\pi^2 n}{2} \left( \frac{1}{\tau} + \beta K \right) + 2 }{\kappa}
		\right) I_\nu(\mu)
		\\
	&= 
		\left( \frac{\tau \beta}{2} 
			+ \frac{1}{\tau} \frac{\pi^2 n}{2\kappa} 
			+ \frac{\pi^2 n \beta K + 4}{2 \kappa} 
		\right) I_\nu(\mu)
		\,, 
\end{aligned}
\end{equation}
and we can optimize over $\tau$ by choosing 
$\tau = \sqrt{ \frac{\pi^2 n}{\beta \kappa} }$, 
which gives us the final constant of 
\begin{equation}
	\sqrt{ \frac{\pi^2 \beta n}{\kappa} } 
	+ \frac{\pi^2 n \beta K + 4}{2 \kappa} 
	\leq 
		\left(\pi + \frac{\pi^2}{2} + 2\right) \frac{\beta K n }{\kappa} 
	\leq 
		\frac{11 \beta K n }{\kappa} 
		\,. 
\end{equation}

\end{proof}













\begin{theorem}[Logarithmic Sobolev Inequality]
\label{thm:lyapunov_log_sobolev_adapted}
Suppose $F$ satisfies 
\cref{asm:app_c3,asm:app_morse,asm:app_unique_min} 
and $d \geq 2$. 
Then for all choices of $a,\beta > 0$ such that 
\begin{equation}
\begin{aligned}
	a^2 
	&\geq 
		\frac{6 K_2 nd}{ C_F^2 } 
		\,, \\
	\beta 
	&\geq
		a^2 
		\max\left( 
			\, \frac{ 4 K_3^2 }{ \lambda_{*}^2 } \,, 
			\, \frac{a^4}{4} (K_3 + 2K_2)^2 \, 
		 \right) \,, 
\end{aligned}
\end{equation}
where $\lambda_*$ is defined in \cref{asm:app_morse}, 
we have that the Markov triple $(M, \nu, \Gamma)$ 
satisfies $\LSI(\alpha)$ with constant 
\begin{equation}
	\frac{1}{\alpha} 
	= 
		\begin{cases}
		 	154 \frac{K_2 n \beta}{\lambda_*^2} \,, 
		 	& \text{ if the global minimum is unique, } \\ 
		 	%
		 	121 \frac{K_2 n \beta^2}{\lambda_*} \,, 
		 	& \text{ otherwise. } 
		\end{cases} 
\end{equation}
\end{theorem}

\begin{proof}

This result follows directly from \cref{prop:poincare_implies_lsi}, 
where we get $\nabla^2 F \geq - K_2 g$ from \cref{asm:app_c3}, 
$\Ric_g = (d-1)g > 0$, and the Poincar\'e constant $\kappa$ from 
\cref{prop:poincare_adapted}. 

\end{proof}























































==> lsi_proof.tex <==

\section{Establishing a Logarithmic Sobolev Inequality - 
Proof of \cref{thm:bm_lsi}}
\label{sec:lsi_proof}

\subsection{Tensorization of LSI and Main Result} 
\label{subsec:tensorization_lsi}

Before we start, we will simplify the structure 
via a quotient. 
First, recalling that the objective $F$ 
for the Burer--Monteiro problem 
is rotationally symmetric. 
Let $G$ be the group of rotation symmetries for $F$, 
then we can view $F$ as a function of the quotient manifold 
$M / G$, which is also a product of spheres. 
Then we can view the Markov triple as a product 
\begin{equation}
	(M, \nu, \Gamma) 
	= ((M / G) \times S^d, 
		\nu_0 \otimes \nu_1, 
		\Gamma_0 \oplus \Gamma_1) 
		\,, 
\end{equation}
where $\nu_0 = \frac{1}{Z_0} e^{-\beta F(x)}$ 
is the quotient Gibbs distribution on $M/G$, 
$\nu_1$ is the uniform distribution on $S^d$, 
$\Gamma_0,\Gamma_1$ are the carr\'{e} du champ operators 
on each respective manifolds. 
Here we also denote $\times$ as the product manifold, 
$\otimes$ as the product measure, 
and $\oplus$ as adding two operators. 

Next we recall the tensorization result of 
logarithmic Sobolev inequalities. 

\begin{proposition}
\citep[Proposition 5.2.7]{bakry2013analysis}
\label{prop:lsi_tensorization_bakry}
Suppose $(M_0, \nu_0, \Gamma_0)$ satisfies $\LSI(\alpha_0)$ 
and $(M_1, \nu_1, \Gamma_1)$ satisfies $\LSI(\alpha_1)$, 
then $(M_0 \times M_1, \nu_0 \otimes \nu_1, \Gamma_0 \oplus \Gamma_1)$ 
satisfies $\LSI( \min(\alpha_0, \alpha_1) )$. 
\end{proposition}

Here we observe that $(S^d, \nu_1, \Gamma)$ 
satisfies $\LSI( \frac{d-1}{\beta} )$ 
using the curvature dimension condition 
\cref{prop:cd_log_sobolev}, 
where we used that $\Ric_{g'} = d-1$ on $S^d$, 
and $g'$ is the Riemannian metric on $S^d$. 
Therefore it is sufficient to show that 
$(M/G, \nu_0, \Gamma_0)$ satisfies $\LSI( \frac{C}{\beta} )$ 
for some constant $C$. 

Then for rest of this section, 
we will without loss of generality 
replace $M/G$ with $M$, 
and assume $F$ is not rotationally symmetric. 
More precisely, 
we will state the main results as follows. 

\begin{assumption}
\label{asm:app_c3}
	$F \in C^3(M)$. In particular, 
	there exist constants $K_1, K_2, K_3 \geq 1$ such that 
	$F$ is $K_1$-Lipschitz, $\grad F$ is $K_2$-Lipschitz, 
	and $\nabla^2 F$ is $K_3$-Lipschitz. 
	Without loss of generality, we can take 
	$\min_{x\in M} F(x) = 0$. 
\end{assumption}

Here we remark that assuming $F$ is $K_1$-Lipschitz 
does not contradict LSI on a compact manifold. 



\begin{assumption}
\label{asm:app_morse}
	$F$ is Morse. 
	In other words, for any critical point $y \in M$, 
	all of the eigenvalues of the Hessian $\nabla^2 F(y)$ 
	are non-zero. 

\end{assumption}

\begin{assumption}
\label{asm:app_unique_min}
	$F$ has a unique local (and hence global) minimum 
	$x^* \in M$. 
\end{assumption}










Before we state the main result, 
we will note most of the constants are specified in 
\cref{subsec:perturb_construction,subsec:lyapunov_regions}. 
Additionally $C_F$ is the Morse constant from 
\cref{lm:morse_grad_est}, 
and $\wt{\kappa}$ is the Poincar\'{e} constant 
from \cref{prop:lyapunov_poincare}. 

\begin{theorem}
[Logarithmic Sobolev Inequality]
\label{thm:lyapunov_log_sobolev}
Suppose $F$ satisfies \cref{asm:app_c3,asm:app_morse,asm:app_unique_min}. 
Then for all choices of $a>0,\beta \geq 1$ such that 
\begin{equation}
\label{eq:lsi_beta_cond}
\begin{aligned}
	a^2 
	&\geq 
		\max\left( 
			\frac{8 K_2^2}{\delta_{\min}^2} 
				[ (n+1)d + 32 ] \,, 
			\frac{2 K_2^2 nd}{ C_F^2 }
			\right)
			\,, \\
	\beta 
	&\geq
		C a^2 (nd)^4 
			\max( \delta_{\min}^{-1}, \delta_{\min}^{-7} ) 
			\max( \wt{\lambda}^{-2}, 1 )
			\max( \lambda_{\min}^{-2}, 1 )
			\max( K_2^{-1}, K_2^6 ) 
			\max( K_3^2, K_3^4 ) \,, 
\end{aligned}
\end{equation}
where $C > 0$ is a universal constant, 
there exists a perturbation $\wt{F}_\beta \in C^3(M)$ 
parameterized by $a, \beta$ such that 
\begin{equation}
	\| \wt{F}_\beta - F \|_\infty \leq \frac{a^2}{\beta} \,, 
\end{equation}
and we have that the Markov triple $(M,\wt{\nu},\Gamma)$ with 
$\wt{\nu}_\beta(dx) = \frac{1}{\wt{Z}} \exp( -\beta \wt{F}_\beta )\,dx$ 
satisfies $\LSI(\wt{\alpha})$ where 
\begin{equation}
	\frac{1}{\wt{\alpha}} 
	= 
		\left[ 
			\sqrt{ 
				\frac{2(1 + \frac{2a^2b}{K_3})}{c \wt{\kappa}} 
			} 
			+ \frac{2 K_2 (1 + \frac{2a^2b}{K_3})}{c \wt{\kappa}} 
			+ \frac{4}{c \wt{\kappa}} 
		\right] 
		+ 
		\beta \left[ 
			\sqrt{ 
				\frac{2}{c} \left( 
				1 + \frac{b}{\wt{\kappa}} 
				\right) 
				}
			+ 
				\frac{K_2}{c} 
				\left( 1 + \frac{2b}{\wt{\kappa}} 
				\right) 
		\right] \,. 
\end{equation}

Furthermore, the unperturbed Markov triple 
$(M,\nu,\Gamma)$ with 
$\nu \propto \exp( -\beta F )$ 
satisfies $\LSI(\alpha)$ with constant 
\begin{equation}
	\alpha 
	= 
		\wt{\alpha} 
		e^{-a^2} 
	= 
		\Omega\left( \frac{1}{\beta} \right) \,, 
\end{equation}
where we use $\Omega(\cdot)$ to show only dependence on $\beta$. 

\end{theorem}





Here we will quickly restate and prove the main result 
\cref{thm:bm_lsi}. 

\begin{theorem}
Let $F:M \to \mathbb{R}$ be the Burer--Monteiro loss function 
defined in \cref{eq:bm_loss_function}, 
and assume $F$ satisfies Assumptions~\ref{asm:bm_morse} and \ref{asm:bm_unique_min}. 
Then we can choose 
\begin{equation}
	\beta \geq \poly( n, d, \Lambda, K_2, K_3 ) \,, 
\end{equation}
such that $(M,\nu,\Gamma)$ with 
$\nu = \frac{1}{Z} e^{-\beta F}$ 
satisfies $\LSI(\alpha)$, 
and $\alpha$ is lower bounded by 
\begin{equation}
	\alpha \geq \frac{C}{\beta} \,, 
\end{equation}
where the constant $C > 0$ is independent of $\beta$, 
but depends on $n,d,\Lambda,K_2,K_3$. 
\end{theorem}

\begin{proof}

Using the discussion above and \cref{prop:lsi_tensorization_bakry}, 
we have that it is sufficient to establish $\LSI(\alpha)$ 
for the Markov triple $(M/G, \nu_0, \Gamma_0)$. 
This is precisely the result of \cref{thm:lyapunov_log_sobolev}, 
with $\alpha = \wt{\alpha} e^{-a^2}$. 

Therefore the constant $C$ can be written as 
\begin{equation}
	C = \max\left( 
		d-1 \,, \alpha \beta 
	\right) \,,
\end{equation}
and the expression for $\poly( n, d, \Lambda, K_2, K_3 )$ 
can be found in \cref{eq:lsi_beta_cond}. 

\end{proof}






















\subsection{Constructing the Perturbation Around a Single Saddle Point}
\label{subsec:perturb_construction}

In this section, we will attempt to construct 
a perturbed potential function 
$\wt{F}_\beta : M \to \mathbb{R}$ such that 
\begin{equation}
	\| \wt{F}_\beta - F \|_\infty \leq \frac{a^2}{\beta} \,, 
\end{equation}
where $a>0$ is a chosen parameter, 
and the perturbed Markov triple $(M, \wt{\nu}, \Gamma)$ 
with $\wt{\nu} = \frac{1}{\wt{Z}} \exp( -\beta \wt{F}_\beta )$ 
satisfies $\LSI(\alpha)$. 
The construction is adapted from \citet{menz2014poincare} 
to our setting, 
and the LSI will be established using a Lyapunov function 
approach \citep{bakry2008simple,cattiaux2010note}. 
Then we can use the Holley--Stroock perturbation lemma 
\citep{holley1987logarithmic} 
to get that the unperturbed Markov triple 
$(M,\nu,\Gamma)$ satisfies $\LSI( \alpha e^{-a^2} )$. 

We start by defining the set of critical points of $F$ as 
\begin{equation}
	\mathcal{C} := \{ y \in M | \grad F(y) = 0 \} \,, 
\end{equation}
and we also define the set of strict saddle points as 
\begin{equation}
	\mathcal{S} := \{ y \in \mathcal{C} | 
		\lambda_{\max}(\nabla^2 F_y) > 0 \,, 
		\lambda_{\min}(\nabla^2 F_y) < 0 
		\} \,, 
\end{equation}
where $\lambda_{\max}, \lambda_{\min}$ 
denote the maximum and minimum eigenvalues. 

In the rest of this subsection, 
we will construct a function $\wt{F}_\beta$ such that 
$\wt{F}_\beta = F$ when 
$d_g(x, \mathcal{S}) > \mathcal{O}(\beta^{-1})$, 
and that $| \wt{F}_\beta - F | \leq \mathcal{O}(\beta^{-1})$. 
Since we assumed $F$ is Morse in \cref{asm:app_morse}, 
and $M$ is compact, 
we have that $\mathcal{C}$ and $\mathcal{S}$ are both finite, 
and each critical point is non-degenerate. 
Therefore without loss of generality, 
we will fix a single $y \in \mathcal{S}$ 
and study this construction individually. 
The fully general case will be specified in 
\cref{subsec:lyapunov_regions}. 

Let $(\lambda_i, u_i)_{i=1}^{nd}$ be the eigenvalues 
and eigenvector pairs of $\nabla^2 F(y)$, 
such that $(u_i)_{i=1}^{nd}$ forms an orthonormal basis 
on $T_y M$. 
Then there exists an $\ell \in [nd]$ 
such that we can separate 
the positive and negative eigenvalues 
\begin{equation}
	\lambda_1 \leq \lambda_2 \leq \cdots 
	\leq \lambda_\ell 
	< 0 < \lambda_{\ell +1 }
	\leq \cdots \leq \lambda_{nd} \,. 
\end{equation} 

Using these, we will define a parameter $\delta > 0$
\begin{equation}
\label{eq:perturb_delta_choice}
	\delta := \begin{cases}
		\min\left\{ \lambda_{\ell + 1} \,, 
			|\lambda_\ell| \right \} \,, 
		& \text{ if } nd \leq 2\ell \,, \\
		\min \left\{ \lambda_{\ell + 1} \,, 
			|\lambda_\ell| \,, 
			\frac{1}{2(nd - 2\ell)} \sum_{i = 1}^\ell |\lambda_i| 
		\right\} 
		&\text{ if } nd > 2\ell \,, 
	\end{cases}
\end{equation}
such that this implies the parameter $\wt{\delta} > 0$
\begin{equation}
\label{eq:delta_tilde_defn}
	\wt{\delta} 
	:= (2\ell - nd) \delta 
		+ \sum_{i = 1}^\ell | \lambda_i | 
	\geq \frac{1}{2} \sum_{i=1}^\ell | \lambda_i | 
	> 0 \,. 
\end{equation}


Let $\log_y:M \to T_y M$ 
be the inverse of $\exp_y:T_y M \to M$, 
which is well-defined outside of the cut locus. 
Then we will define a scaled geodesic distance 
$d_{\delta,y}:M \to \mathbb{R}$ as 
\begin{equation}
\label{eq:delta_norm}
	d_{\delta, y}(x)^2 
	:= 
		\sum_{i=1}^\ell \frac{\delta}{2} 
		\langle \log_y(x), u_i \rangle_g^2 
	+ 
		\sum_{i=\ell+1}^{nd} \frac{ \lambda_i - \delta }{2} 
		\langle \log_y(x), u_i \rangle_g^2 \,. 
\end{equation}

Let $d_y(x) := d_g(x,y)$ be 
the classical geodesic distance between $x,y$, 
we observe that we can write 
\begin{equation}
	d_y(x)^2 
	= |\log_y (x)|_g^2 
	= \sum_{i=1}^{nd} \langle \log_y(x), u_i \rangle_g^2 \,, 
\end{equation}
and therefore we can derive the following estimates 
\begin{equation}
\label{eq:delta_norm_est}
	\frac{\delta}{2} d_y(x)^2 
	\leq d_{\delta, y}(x)^2 
	\leq \frac{\lambda_{\max} - \delta}{2} d_y(x)^2 
	\leq \frac{\lambda_{\max}}{2} d_y(x)^2 \,. 
\end{equation}

We will construct a desired smooth cutoff function 
$\xi:\mathbb{R}^+ \to \mathbb{R}$. 

\begin{lemma}
[A Special Smooth Cutoff Function]
For all constants $a,\beta > 0$, 
there exists a function $\xi : [0,\infty) \to \mathbb{R}$ 
satisfying all of the following properties 
\begin{enumerate}
	\item $\xi \in C^\infty([0,\infty), \mathbb{R})$ \,, 
	\item $\xi'(r) = -1$ for $r \leq \frac{1}{4} \frac{a^2}{\beta}$ \,, 
	\item $\xi'(r) \in [-1,0]$ for $r \geq \frac{1}{4} \frac{a^2}{\beta}$ \,, 
	\item $\xi(r) = 0$ for $r \geq \frac{a^2}{\beta}$ \,, 
	\item $\xi(r) \in [0, \frac{a^2}{\beta}]$ 
		for some constant $C_\xi>0$ independent of $a, \beta$ \,, 
	\item $|\xi''(r)| \leq 4 \frac{\beta}{a^2}$ 
		for some constant $C_\xi>0$ independent of $a, \beta$ \,. 
\end{enumerate}
\end{lemma}

The full proof of this construction can be found in 
\cref{sec:app_misc_tech} \cref{lm:smooth_cutoff}. 
Finally this allows us to define the perturbation 
\begin{equation}
	\wt{F}_\beta(x) 
	:= F(x) 
	+ \xi\left( d_{\delta,y}(x)^2 \right) \,, 
\end{equation}
and note that $a, \beta > 0$ remain two parameters 
that can be chosen later. 
Furthermore, we will later use the same construction 
around each $y \in \mathcal{S}$, 
and choose each parameter $\delta, a, \beta > 0$ 
as a function of $y$. 



















\subsection{Technical Estimates on Laplacian and Gradient}



Before we start this subsection, 
we note that many of the technical estimates 
using Riemannian normal coordinates can be found in 
\cref{subsec:app_normal_sd}. 



\begin{lemma}
\label{lm:perturb_laplacian_upper_bound}
Suppose $F$ satisfies \cref{asm:app_c3,asm:app_morse,asm:app_unique_min}. 
Then for all choices of $a,\beta > 0$ such that 
\begin{equation}
	\frac{a^2}{\beta} 
	\leq 
		\min \left( 
			\frac{ \delta }{ 4 d \sqrt{n} } \,, 
			\frac{3 \delta^{3/2}}{ 2 \sqrt{K_2} n d } \,, 
			2 K_2 
			\right) \,, 
\end{equation}
we have that 
\begin{equation}
	\Delta \wt{F}_\beta(x) \leq K_2 (d + 32) \,, 
		\quad \forall \, d_{\delta,y}(x) \in 
		\left[ \frac{a}{ 2 \sqrt{\beta} }, \frac{a}{ \sqrt{\beta} } \right] 
		\,. 
\end{equation}
\end{lemma}

\begin{proof}

Before we start, we observe that 
$d_{\delta, y}(x)^2 \leq \frac{a^2}{\beta} 
\leq 2 K_2$ implies $|x| \leq \frac{\pi}{2}$ 
using \cref{eq:delta_norm_est}. 

We start by computing the Laplacian directly 
\begin{equation}
	\Delta \wt{F}_\beta(x) 
	= \Delta F(x) 
		+ \xi''\left( d_{\delta,y}(x)^2 \right) 
			\left| \grad d_{\delta,y}(x)^2 \right|_g^2 
		+ \xi'\left( d_{\delta,y}(x)^2 \right) 
			\Delta \left( d_{\delta,y}(x)^2 \right) \,. 
\end{equation}

Here we first observe that 
$\xi'\left( d_{\delta,y}(x)^2 \right) \leq 0$ 
and we also claim that 
$\Delta \left( d_{\delta,y}(x)^2 \right) \geq 0$. 
To see this, we expand the Laplacian term 
in normal coordinates 
\begin{equation}
	\Delta d_{\delta, y}(x)^2 
	= \sum_{i=1}^{nd} c_i \Delta 
		\frac{1}{2} \langle x, u_i \rangle^2 \,, 
\end{equation}
where $c_i = \delta$ when $i \leq \ell$ 
and $c_i = \lambda_i - \delta$ otherwise. 
Then we can use \cref{lm:grad_laplacian_prod_approx} to get 
\begin{equation}
	\left| \Delta \frac{1}{2} \langle x, u_i \rangle^2 
		- 1 
	\right| 
	\leq 2 d \sqrt{n} |x|^2 \,, 
\end{equation}
therefore it is sufficient to have $2 d \sqrt{n} |x|^2 \leq 1$, 
which is satisfied when 
$ \frac{a^2}{\beta} \leq \frac{ \delta }{ 4 d \sqrt{n} }$. 
As a result, we can drop the last negative term 
for an upper bound. 

Next we will expand the gradient term similarly 
\begin{equation}
	\grad d_{\delta, y}(x)^2 
	= \sum_{i=1}^{nd} c_i \grad \frac{1}{2} \langle x , u_i \rangle^2 
		\,, 
\end{equation}
then using \cref{lm:grad_laplacian_prod_approx} 
we can write 
\begin{equation}
	\left| 
		\grad d_{\delta, y}(x)^2 
		- \sum_{i=1}^{nd} c_i \langle x , u_i \rangle u_i 
	\right|_g 
	\leq 
		\sum_{i=1}^nd |c_i| \frac{1}{3} |x|^3 
	\leq 
		\frac{ \lambda_{\max} n d }{3} |x|^3 
		\,. 
\end{equation}

Using the triangle inequality, we can write 
\begin{equation}
	\left| 
		\grad d_{\delta, y}(x)^2 
	\right|_g 
	\leq 
		\left| 
			\sum_{i=1}^{nd} c_i \langle x , u_i \rangle u_i 
		\right|_g 
		+ \frac{ \lambda_{\max} n d }{3} |x|^3 \,, 
\end{equation}
then we can use $(a+b)^2 \leq 2 a^2 + 2 b^2$ to write 
\begin{equation}
	\left| 
		\grad d_{\delta, y}(x)^2 
	\right|_g^2 
	\leq 
		2 \left| 
			\sum_{i=1}^{nd} c_i \langle x , u_i \rangle u_i 
		\right|_g^2 
		+ \frac{ 2 (\lambda_{\max} n d)^2 }{9} |x|^6 \,. 
\end{equation}

Since $(u_i)_{i=1}^{nd}$ form an orthonormal basis, 
we can write 
\begin{equation}
	\left| 
		\sum_{i=1}^{nd} c_i \langle x , u_i \rangle u_i 
	\right|_g^2 
	= 
		\sum_{i=1}^{nd} c_i^2 \langle x , u_i \rangle^2 
	\leq 
		2 \lambda_{\max} d_{\delta, y}(x)^2 \,. 
\end{equation}

Furthermore, we will also use the estimates on $d_{\delta,y}(x)$
from \cref{eq:delta_norm_est} to write 
\begin{equation}
	|x|^2 
	= d_{y}(x)^2 
	\leq \frac{2}{\delta} d_{\delta, y}(x)^2 
	\leq \frac{2 a^2}{ \delta \beta } \,, 
\end{equation}
in combination with the fact that $\xi'' \leq \frac{4\beta}{a^2}$ 
from \cref{lm:smooth_cutoff}, 
we can finally write 
\begin{equation}
\begin{aligned}
	\Delta \wt{F}_\beta(x) 
	&\leq 
		\Delta F(x) + \frac{4\beta}{a^2} 
		\left[ 4 \lambda_{\max} \frac{a^2}{\beta} 
			+ \frac{16 (\lambda_{\max} n d)^2 }{ \delta^3 } 
				\frac{a^6}{\beta^3}
		\right] 
		\\ 
	&= 
		\Delta F(x) 
		+ 16 \lambda_{\max} \left[ 
			1 + \frac{ 4 \lambda_{\max} n^2 d^2 }{ \delta^3 } 
				\frac{a^4}{\beta^2} 
			\right] \,. 
\end{aligned}
\end{equation}

To get the desired result, 
we will use the facts that $\Delta F \leq K_2 d$, 
$\lambda_{\max} \leq K_2$, 
and the choice of 
$\frac{a^2}{\beta} \leq \frac{3 \delta^{3/2}}{ 2 \sqrt{K_2} n d }$ 
to write 
\begin{equation}
	\Delta \wt{F}_\beta(x) 
	\leq 
		K_2 d 
		+ 16 K_2 \left[ 
			1 + \frac{ 4 K_2 n^2 d^2 }{ \delta^3 } 
				\frac{a^4}{\beta^2} 
			\right] 
	\leq 
		K_2 (d + 32) \,. 
\end{equation}

\end{proof}













Before we start the next lemma, 
we will define a vector field in the normal coordinates 
centered at $y \in M$ as follows 
\begin{equation}
	H_i(x) \de_i := g^{ik} \de_k \de_j F(0) x_j \de_i \,, 
\end{equation}
and observe that loosely speaking, 
$H(x)$ behaves like $\nabla^2 F(0)^\sharp [x]$, 
i.e. gradient of the local quadratic approximation of $F(x)$, 
where $\sharp$ is the musical isomorphism that raises an index 
\citep{lee2019riemann}. 

\begin{lemma}
\label{lm:perturb_additional_lower_bounds}
Suppose $F$ satisfies 
\cref{asm:app_c3,asm:app_morse,asm:app_unique_min}. 
Then for all choices of $a,\beta > 0$ such that 
\begin{equation}
	\frac{a^2}{\beta} 
	\leq 
		\min \left( \frac{ \delta^2 }{ 2 nd K_2 } \,, 
			2 K_2 
		\right) 
		\,, 
\end{equation}
then we have the following bounds 
\begin{equation}
\begin{aligned}
	| \grad F(x) - H(x) |_g 
		&\leq 
			\frac{\pi^2}{4} \left( K_3 + 4\pi nd K_2 \right) 
			|x|^2 
			\,, \\ 
		&\leq 
			\frac{\pi^2}{2} \frac{ K_3 + 4\pi nd K_2 }{\delta} 
			d_{\delta, y}(x)^2 
		\,, \\ 
	| \grad F(x) |_g^2 
		&\geq 
		| H(x) |_g^2 
		- \frac{ 100 K_3^2 + 8700 n^2 d^2 K_2^2 }{ \delta^{3/2} } 
			d_{\delta,y}(x)^3 \,, \\ 
	| \grad \xi( d_{\delta,y}(x)^2 ) |_g^2 
		&\leq | \grad \xi( d_{\delta,y}(x)^2 ) |^2 
		\leq 
		4 K_2 d_{\delta,y}(x)^2 \,, \\
	\langle \grad F(x), \grad \xi ( d_{\delta,y}(x)^2 ) \rangle_g 
		&\geq 
		\langle H(x), \grad \xi ( d_{\delta,y}(x)^2 ) \rangle_g 
			- \pi^2 \frac{ (K_3 + 4\pi nd K_2) \sqrt{K_2} }{ \delta }  
			d_{\delta,y}(x)^3 \,. 
\end{aligned}
\end{equation}
\end{lemma}

\begin{proof}

\noindent
\textbf{Estimate 1.}

We start by doing a quick calculation on 
\begin{equation}
	|g^{ik} u^k \de_i|_g^2 
	= g^{ik} u^k g_{ij} g^{jk'} u^{k'} 
	= g^{ik} u^i u^k \,, 
\end{equation}
and since $g^{ik}$ has eigenvalues $1$ and $\frac{|x|^2}{\sin^2(|x|)}$, 
we have the following two sided estimates 
when $|x| \leq \frac{\pi}{2}$ 
\begin{equation}
\label{eq:normal_metric_two_est}
	|u^i \de_i|_g
	\leq |g^{ik} u^k \de_i|_g 
	\leq \frac{\pi^2}{4} |u^i \de_i|_g \,. 
\end{equation}

This allows us to write 
\begin{equation}
	| \grad F(x) - H(x) |_g 
	= 
		| g^{ik} ( \de_k F - \de_k \de_j F(0) x_j ) \de_i |_g 
	\leq 
		\frac{\pi^2}{4} |(\de_k F - \de_k \de_j F(0) x_j) \de_k |_g 
		\,. 
\end{equation}

We will next use the intermediate value theorem on $\mathbb{R}^d$, 
which implies there exists an $\hat{x}$ along 
the line between $0$ and $x$ such that 
\begin{equation}
	\de_k F(x) = \de_k F(0) + \de_j \de_k F( \hat{x} ) x_j \,, 
\end{equation}
and since $\de_j F(0) = 0$, we also have 
\begin{equation}
	\frac{\pi^2}{4} |(\de_k F - \de_k \de_j F(0) x_j) \de_k |_g 
	\leq 
		\frac{\pi^2}{4} |(\de_j \de_k F( \hat{x} ) x_j - \de_k \de_j F(0) x_j) 
						\de_k |_g 
		\,. 
\end{equation}

Here we will recall the local coordinate formula 
for the Hessian 
\begin{equation}
	\nabla^2 F(x) 
	= ( \de_i \de_j F - \Gamma_{ij}^k \de_k F) \, 
		dx^i \otimes dx^j \,, 
\end{equation}
and using the fact that $\Gamma_{ij}^k(0) = 0$ for normal coordinates, 
we will also get that 
\begin{equation}
	\frac{\pi^2}{4} |(\de_j \de_k F( \hat{x} ) x_j - \de_k \de_j F(0) x_j) 
					\de_k |_g 
	\leq 
		\frac{\pi^2}{4} \left( 
			|\nabla^2 F(\hat{x}) - \nabla^2 F(0)|_g 
			+ |\Gamma_{ij}^k(\hat{x}) \de_k F(\hat{x}) \de_i |_g 
			\right) 
			|x|_g \,. 
\end{equation}

Using the fact that $\nabla^2 F$ is $K_3$-Lipschitz, 
we can write 
\begin{equation}
	|\nabla^2 F(\hat{x}) - \nabla^2 F(0)|_g 
	\leq 
		K_3 |\hat{x}| 
	\leq 
		K_3 |x| \,, 
\end{equation}
and using the two sided estimates on $|g^{ik}u^k \de_k|_g$ 
and \cref{lm:christoffel_bound}, 
we can write 
\begin{equation}
	|\Gamma_{ij}^k(\hat{x}) \de_k F(\hat{x}) \de_i |_g 
	\leq 
		nd \, |\Gamma_{ij}^k(\hat{x})| \, 
		| g^{ik} \de_k F(\hat{x}) \de_i |_g 
	\leq 
		nd \, 8|\hat{x}| \, 
		K_2 |\hat{x}| 
	\leq 
		4\pi nd K_2 |x| \,, 
\end{equation}
where we used the fact that $\grad F$ is $K_2$-Lipschitz, 
and that $|x| \leq \frac{\pi}{2}$. 
Observe that $d_{\delta, y}(x)^2 \leq \frac{a^2}{\beta} 
\leq 2 K_2$ implies $|x| \leq \frac{\pi}{2}$ 
using \cref{eq:delta_norm_est}. 

Putting everything together, 
we have the first estimate 
\begin{equation}
	| \grad F(x) - H(x) |_g 
	\leq 
		\frac{\pi^2}{4} \left( K_3 + 4\pi nd K_2 \right) |x|^2 
	\leq 
		\frac{\pi^2}{2} \frac{ K_3 + 4\pi nd K_2 }{\delta} 
		d_{\delta, y}(x)^2 \,, 
\end{equation}
where we used the estimate \cref{eq:delta_norm_est}. 





\vspace{0.2cm}
\noindent
\textbf{Estimate 2.}

Next we will directly compute 
\begin{equation}
\begin{aligned}
	| \grad F(x) |_g^2 
	&= 
		|H(x)|_g^2 + | \grad F(x) - H(x) |_g^2 
		+ 2 \langle H(x), \grad F(x) - H(x) \rangle_g \\ 
	&\geq 
		|H(x)|_g^2 - | \grad F(x) - H(x) |_g^2 
		- 2 | H(x) |_g \, | \grad F(x) - H(x) |_g \,, 
\end{aligned}
\end{equation}
where we used the Cauchy-Schwarz inequality. 

Here we observe that using the two sided estimate 
\cref{eq:normal_metric_two_est}, 
we can write 
\begin{equation}
	| H(x) |_g 
	\leq 
		\frac{\pi}{2} | \de_k \de_i F(0) x^i \de_k | 
	\leq 
		\frac{\pi}{2} K_2 |x| \,, 
\end{equation}
and additionally using the first estimate we can get 
\begin{equation}
	| \grad F(x) |_g^2 
	\geq 
		| H(x) |_g^2 
		- \frac{\pi^4}{16} \left( K_3 + 4\pi nd K_2 \right)^2 |x|^4 
		- \pi K_2 |x| 
			\frac{\pi^2}{4} \left( K_3 + 4\pi nd K_2 \right) |x|^2 
			\,. 
\end{equation}

Using the inequality $(a+b)^2 \leq 2a^2 + 2b^2$ 
and the fact that $|x| \leq \frac{\pi}{2}$, 
we can write 
\begin{equation}
	| \grad F(x) |_g^2 
	\geq 
		| H(x) |_g^2 
		- \left[ 
			\frac{ \pi^5 }{16} K_3^2 
			+ \pi^7 n^2 d^2 K_2^2 
			+ \frac{ \pi^3 }{2} K_2^2 
			+ \frac{ \pi^3 }{2} K_3^2 
			+ 4\pi^2 nd K_2 
		\right] 
			\left( \frac{2}{\delta} \right)^{3/2} 
			d_{\delta,y}(x)^3 \,, 
\end{equation}
and here we will use the fact that $n,d \geq 1$ 
and round up all universal constants to 
get the desired bound 
\begin{equation}
	| \grad F(x) |_g^2 
	\geq 
		| H(x) |_g^2 
		- 
		\frac{ 100 K_3^2 + 8700 n^2 d^2 K_2^2 }{ \delta^{3/2} } 
			d_{\delta,y}(x)^3 \,. 
\end{equation}









\vspace{0.2cm}
\noindent
\textbf{Estimate 3.}

We start by using the fact that $|u|_g \leq |u|$ 
and expand out the terms 
\begin{equation}
	| \grad \xi( d_{\delta,y}(x)^2 ) |_g 
	\leq 
		| \xi' |^2 \, 
		\left| \sum_{i=1}^{nd} c_i \langle x, u_i \rangle 
			\grad \langle x, u_i \rangle  
		\right|^2 
	\leq 
		\sum_{i,j=1}^{nd} 
			c_i c_j 
			\langle x, u_i \rangle 
			\langle x, u_j \rangle 
			\langle \grad \langle x, u_i \rangle, 
				\grad \langle x, u_j \rangle  
				\rangle 
\end{equation}
where we denote $c_i = \delta$ or $\lambda_i - \delta$ 
based on the definition \cref{eq:delta_norm}, 
and used the fact that $| \xi' | \leq 1$ 
from the construction in \cref{lm:smooth_cutoff}. 

Next we will use \cref{lm:grad_laplacian_prod_approx} 
to write 
\begin{equation}
	\langle \grad \langle x, u_i \rangle, 
				\grad \langle x, u_j \rangle  
				\rangle 
	\leq 
		\langle u_i, u_j \rangle 
		+ \frac{1}{3} |x|^2 ( |u_i| + |u_j| ) 
		+ \frac{1}{9} |x|^4 
	\leq 
		\delta_{ij}
		+ |x|^2 \,. 
\end{equation}
where we used the facts that $|x| \leq \frac{\pi}{2}$, 
$|u_i| = |u_j| = 1$, 
and rounded up the constant to $1$. 

We return to the original estimate and write 
\begin{equation}
	| \grad \xi( d_{\delta,y}(x)^2 ) |_g 
	\leq 
		\sum_{i=1}^{nd} c_i^2 \langle x, u_i \rangle^2 
		+ \sum_{i,j=1}^{nd} c_i c_j 
			\langle x, u_i \rangle 
			\langle x, u_j \rangle 
			|x|^2 
	\leq 
		2 \lambda_{\max} d_{\delta, y}(x)^2 
		+ nd \lambda_{\max}^2 \frac{4}{\delta^2} 
			d_{\delta, y}(x)^4 \,, 
\end{equation}
where we used the fact that $c_i \leq \lambda_{\max}$, 
Cauchy-Schwarz inequality, 
and the estimates from $\cref{eq:delta_norm_est}$. 

Finally, we will use the fact that $\lambda_{\max} \leq K_2$ 
and the choice of 
\begin{equation}
	d_{\delta, y}(x)^2 
	\leq \frac{a^2}{\beta} 
	\leq \frac{ \delta^2 }{ 2 nd K_2 } \,, 
\end{equation}
this gives us the desired bound of 
\begin{equation}
	| \grad \xi( d_{\delta,y}(x)^2 ) |_g 
	\leq 
		4 K_2 d_{\delta,y}(x)^2 \,. 
\end{equation}

















\vspace{0.2cm}
\noindent
\textbf{Estimate 4.}

We will directly expand the desired object 
and use the Cauchy-Schwarz inequality to write 
\begin{equation}
	\langle \grad F, \grad \xi \rangle_g 
	= 
		\langle H, \grad \xi \rangle_g 
		+ \langle \grad F - H, \grad \xi \rangle_g 
	\geq 
		\langle H, \grad \xi \rangle_g 
		- | \grad F - H |_g \, 
			| \grad \xi |_g \,. 
\end{equation}

Using the first and third estimates from the current lemma, 
we can write 
\begin{equation}
\begin{aligned}
	\langle \grad F, \grad \xi \rangle_g 
	&\geq 
		\langle H, \grad \xi \rangle_g 
		- 
		\frac{\pi^2}{2} \frac{ K_3 + 4\pi nd K_2 }{\delta} 
			d_{\delta, y}(x)^2 \, 
		2 \sqrt{ K_2 } 
			d_{\delta, y}(x) \\
	&= 
		\langle H, \grad \xi \rangle_g 
		- \pi^2 \frac{ (K_3 + 4\pi nd K_2) \sqrt{K_2} }{ \delta } 
			d_{\delta, y}(x)^3 \,, 
\end{aligned}
\end{equation}
which is the desired bound. 











\end{proof}




































\begin{lemma}
\label{lm:perturb_grad_lower_bound}
Suppose $F$ satisfies 
\cref{asm:app_c3,asm:app_morse,asm:app_unique_min}. 
Then for all choices of $a,\beta > 0$ such that 
\begin{equation}
	\frac{a^2}{\beta} 
	\leq 
		\min \left( 
			\frac{\delta^2}{ 2 nd K_2 } \,, 
			2K_2 \,, 
			\frac{ \delta^4 }{ 16 K_2^2 } 
			\left[ 
				\frac{ 100 K_3^2 + 8710 (n d K_2)^2 }{ \delta^{3/2} }
				+ \frac{ 2\pi^2 (K_3 + 4\pi nd K_2) K_2^{1/2} }{ \delta }
				+ \frac{\pi K_2}{\delta^{1/2}} 
			\right]^{-2} 
		\right) 
		\,, 
\end{equation}
we have the following bound 
\begin{equation}
	| \grad \wt{F}_\beta(x) |_g^2 
	\geq 
		\frac{\delta^2}{4 K_2 }
		\frac{a^2}{\beta} \,, 
		\quad \forall \, d_{\delta,y}(x) \in 
		\left[ \frac{a}{2 \sqrt{\beta}}, \frac{a}{\sqrt{\beta}} \right] 
		\,. 
\end{equation}
\end{lemma}

\begin{proof}

We will start by directly expanding the gradient norm term 
and use \cref{lm:perturb_additional_lower_bounds} 
to approximate it as 
\begin{equation}
\begin{aligned}
	| \grad \wt{F}_\beta(x) |_g^2 
	&= 
		| \grad F(x) |_g^2 
		+ | \grad \xi( d_{\delta,y}(x)^2 ) |_g^2 
		+ 2 \langle \grad F(x), 
				\grad \xi( d_{\delta,y}(x)^2 )
			\rangle_g \\ 
	&\geq 
		| H(x) |_g^2 
		+ | \grad \xi( d_{\delta,y}(x)^2 ) |_g^2 
		+ 2 \langle H(x), 
				\grad \xi( d_{\delta,y}(x)^2 )
			\rangle_g 
		- (C_2 + 2 C_4) d_{\delta,y}(x)^3 \,, 
\end{aligned}
\end{equation}
where $C_2, C_4 > 0$ are constants from 
the second and fourth estimates of 
\cref{lm:perturb_additional_lower_bounds} 
which we will fill in later. 

Here we will make a few more approximations 
to replace all Riemannian inner products 
with an eigendecomposition sum, 
starting with $|H(x)|_g^2$ 
\begin{equation}
	| H |_g^2 
	= 
		g^{ij} 
		( \de_i \de_k F(0) x_k ) 
		( \de_j \de_{k'} F(0) x_{k'} ) 
	\geq 
		| \de_i \de_k F(0) x_k \de_i |^2 
	= 
		\sum_{i=1}^{nd} 
		\lambda_i^2 \langle x, u_i \rangle^2 \,. 
\end{equation}

Next we will use \cref{lm:inner_product_approx} to write 
\begin{equation}
\begin{aligned}
	| \grad \xi( d_{\delta,y}(x)^2 ) |_g^2 
	&\geq 
		| \grad \xi( d_{\delta,y}(x)^2 ) |^2 
		- \frac{1}{3} |x|^2 | \grad \xi( d_{\delta,y}(x)^2 ) |^2 
		\\ 
	&\geq 
		| \grad \xi( d_{\delta,y}(x)^2 ) |^2 
		- \frac{1}{3} \frac{\pi}{2} \sqrt{ \frac{2}{\delta} } 
			d_{\delta, y}(x) \, 
			4 K_2 d_{\delta, y}(x)^2 
			\\
	&\geq 
		| \grad \xi( d_{\delta,y}(x)^2 ) |^2 
		- \frac{ \pi K_2 }{ \delta^{1/2} } 
			d_{\delta, y}(x)^3 \,, 
\end{aligned}
\end{equation}
where we used the fact that $|x| \leq \frac{\pi}{2}$, 
the third estimate from $\cref{lm:perturb_additional_lower_bounds}$, 
the norm estimates from \cref{eq:delta_norm_est}, 
and rounded up $2 \sqrt{2} / 3 < 1$. 

Here we will further expand the squared norm term 
and use \cref{lm:grad_laplacian_prod_approx} 
to write 
\begin{equation}
\begin{aligned}
	| \grad \xi( d_{\delta,y}(x)^2 ) |^2 
	&= 
		|\xi'|^2 \sum_{i,j=1}^{nd} c_i c_j 
			\langle x, u_i \rangle \langle x, u_j \rangle 
			\langle \grad \langle x, u_i \rangle, 
				\grad \langle x, u_j \rangle 
				\rangle 
				\\ 
	&\geq 
		|\xi'|^2 \sum_{i=1}^{nd} 
			c_i^2 \langle x, u_i \rangle^2 
		- \sum_{i,j=1}^{nd} c_i c_j 
			|x|^2 \, 
			\left( \frac{2}{3} + \frac{\pi^2}{36} 
			\right) |x|^2 
			\\ 
	&\geq 
		|\xi'|^2 \sum_{i=1}^{nd} 
			c_i^2 \langle x, u_i \rangle^2 
		- nd K_2^2 |x|^4 
		\\ 
	&\geq 
		|\xi'|^2 \sum_{i=1}^{nd} 
			c_i^2 \langle x, u_i \rangle^2 
		- \frac{5 nd K_2^2}{ \delta^{3/2} } d_{\delta,y}(x)^3 \,, 
\end{aligned}
\end{equation}
where we used the facts that $|\xi'| \leq 1$ 
from \cref{lm:smooth_cutoff}, 
$c_i \leq \lambda_{\max} \leq K_2$, 
$|x| \leq \frac{\pi}{2}$, 
the norm estimates from \cref{eq:delta_norm_est}, 
and rounded up the constants. 




For the inner product term, 
we will that the metric in the inner product actually cancels 
with the inverse metric in $H$, 
so we can write 
\begin{equation}
	2 \langle H(x), 
			\grad \xi( d_{\delta,y}(x)^2 )
		\rangle_g 
	= 
		2 \left\langle \de_i \de_j F(0) x_j \de_i , 
			\xi' \sum_{i=1}^{nd} \langle x, u_i \rangle 
				\grad \langle x, u_i \rangle 
		\right\rangle \,. 
\end{equation}

Here we will use the eigendecomposition to write 
\begin{equation}
	\de_i \de_j F(0) x_j \de_i 
	= \sum_{i=1}^{nd} \lambda_i 
		\langle x, u_i \rangle u_i \,, 
\end{equation}
and similarly recall that 
$| \grad \langle x, u_i \rangle - u_i | 
\leq \frac{1}{3}|x|^2$ 
from \cref{lm:grad_laplacian_prod_approx}, 
this allows us to write 
\begin{equation}
\begin{aligned}
	& \quad 
		2 \langle \de_i \de_j F(0) x_j \de_i , 
			\xi' \sum_{i=1}^{nd} \langle x, u_i \rangle 
				\grad \langle x, u_i \rangle 
		\rangle 
		\\ 
	&= 2 \sum_{i=1}^{nd} \lambda_i \xi' c_i 
		\langle x, u_i \rangle^2 
		+ 
		\left\langle \de_i \de_j F(0) x_j \de_i \,, 
			\xi' \sum_{i=1}^{nd} c_i \langle x, u_i \rangle 
			( u_i - \grad \langle x, u_i \rangle )
		\right\rangle 
		\\ 
	&\geq 
		2 \sum_{i=1}^{nd} \lambda_i \xi' c_i 
		\langle x, u_i \rangle^2 
		- 
		| \de_i \de_j F(0) x_j \de_i | \, 
		\sum_{i=1}^{nd} |\xi'| \, c_i |x| \, \frac{1}{3} |x|^2 
		\\ 
	&\geq 
		2 \sum_{i=1}^{nd} \lambda_i \xi' c_i 
		\langle x, u_i \rangle^2 
		- 
		K_2 |x| \, 
		\frac{ nd K_2 }{3} |x|^3 
		\\ 
	&\geq 
		2 \sum_{i=1}^{nd} \lambda_i \xi' c_i 
		\langle x, u_i \rangle^2 
		- 
		\frac{ 2 nd K_2^2}{ \delta^{3/2} } d_{\delta,y}(x)^3 
		\,, 
\end{aligned}
\end{equation}
where we used the Cauchy-Schwarz and triangle inequalities, 
the fact that $c_i \leq \lambda_{\max} \leq K_2$, 
that $|\xi'| \leq 1$ from the construction in 
\cref{lm:smooth_cutoff}, 
that $|x| \leq \frac{\pi}{2}$, 
the norm estimates from \cref{eq:delta_norm_est}, 
and rounded up the constant. 

Putting all the terms together, 
we have 
\begin{equation}
	| \grad \wt{F}_\beta(x) |_g^2 
	\geq 
		\sum_{i=1}^{nd} \big( 
			\lambda_i^2 + c_i^2 |\xi'|^2
			+ 2 \lambda_i c_i \xi' 
			\big) \langle x, u_i \rangle^2 		
		- \left( 
			C_2 + 2C_4 + \frac{\pi K_2}{ \delta^{1/2} } 
			+ \frac{ 7 nd K_2^2 }{ \delta^{3/2} } 
		\right) 
			d_{\delta,y}(x)^3 \,. 
\end{equation} 

At this point, we will study the coefficients in the sum, 
which we can rewrite as 
\begin{equation}
	\lambda_i^2 + c_i^2 |\xi'|^2
			+ 2 \lambda_i c_i \xi' 
	= 
		( \lambda_i + \xi' c_i )^2 \,. 
\end{equation}

For $i \leq \ell$, we have that $\lambda_i < 0$, 
and $c_i = \delta$, 
therefore we can write 
\begin{equation}
	( \lambda_i + \xi' c_i )^2 
	= ( |\lambda_i| + |\xi'| \delta )^2 
	\geq \delta^2 \,, 
\end{equation}
where we used the fact that $|\lambda_i| \geq \delta$ 
for $i \leq \ell$. 

On the other hand, when $i > \ell$, 
we have that $\lambda_i > 0$, 
therefore we write 
\begin{equation}
	( \lambda_i + \xi' c_i )^2 
	= ( \lambda_i - |\xi'| ( \lambda - \delta ) )^2 
	\geq \delta^2 \,. 
\end{equation}

This gives us 
\begin{equation}
\begin{aligned}
	| \grad \wt{F}_\beta(x) |_g^2 
	&\geq 
		\sum_{i=1}^{nd} 
			\delta^2 
			\langle x, u_i \rangle^2 
		- C d_{\delta,y}(x)^3 
		\\ 
	&= 
		\delta^2 |x|^2 
		- C d_{\delta,y}(x)^3 
		\\ 
	&\geq 
		\frac{2 \delta^2}{ K_2 } d_{\delta, y}(x)^2 
		- C d_{\delta,y}(x)^3 \,, 
\end{aligned}
\end{equation}
where we will fill in the constant $C>0$ later, 
and we used the norm estimate from \cref{eq:delta_norm_est}. 

At this point, we will use the upper and lower bound of 
$d_{\delta, y}(x)^2 \in [ \frac{a^2}{4\beta}, \frac{a^2}{\beta} ]$ 
to write 
\begin{equation}
	| \grad \wt{F}_\beta(x) |_g^2 
	\geq 
		\frac{2 \delta^2}{ K_2 } \frac{a^2}{4\beta} 
		- C \frac{a^3}{\beta^{3/2}} \,, 
\end{equation}
therefore to get the desired result, we will choose 
\begin{equation}
\begin{aligned}
	\frac{a}{\sqrt{\beta}} 
	&\leq 
		\frac{\delta^2}{ 4 C K_2 } \\ 
	&= 
		\frac{ \delta^2 }{ 4 K_2 } 
		\left[ C_2 + 2 C_4 + \frac{\pi K_2}{\delta^{1/2}} 
			+ \frac{ 7 nd K_2^2 }{ \delta^{3/2} } 
		\right]^{-1} 
		\\ 
	&= \frac{ \delta^2 }{ 4 K_2 } 
		\left[ 
			\frac{ 100 K_3^2 + 8700 (n d K_2)^2 }{ \delta^{3/2} }
			+ \frac{ 2\pi^2 (K_3 + 4\pi nd K_2) K_2^{1/2} }{ \delta }
			+ \frac{\pi K_2}{\delta^{1/2}} 
			+ \frac{ 7 nd K_2^2 }{ \delta^{3/2} } 
		\right]^{-1} 
		\\
	&\leq 
		\frac{ \delta^2 }{ 4 K_2 } 
		\left[ 
			\frac{ 100 K_3^2 + 8707 (n d K_2)^2 }{ \delta^{3/2} }
			+ \frac{ 2\pi^2 (K_3 + 4\pi nd K_2) K_2^{1/2} }{ \delta }
			+ \frac{\pi K_2}{\delta^{1/2}} 
		\right]^{-1} 
		\,, 
\end{aligned}
\end{equation}
where we used the fact that $n,d \geq 1$, 
and this gives us the desired bound of 
\begin{equation}
	| \grad \wt{F}_\beta(x) |_g^2 
	\geq 
		\frac{\delta^2}{ 4 K_2 } \,. 
\end{equation}







\end{proof}

























\subsection{Computing the Lyapunov Condition in Different Regions}
\label{subsec:lyapunov_regions}

In this subsection, 
we will attempt to show that after a perturbation 
around each saddle point, 
the new potential function satisfies a Lyapunov condition 
of the type 
\begin{equation}
	\frac{1}{2} \Delta \wt{F}_\beta 
	- \frac{\beta}{4} | \grad \wt{F}_\beta |_g^2 
	\leq 
		- \theta + b \mathds{1}_U \,, 
\end{equation}
where $\theta, b > 0$ are constants to be specified, 
and $U$ is a neighbourhood around the global minimum $x^*$. 

To this goal, we will make precise the perturbation on $F$. 
Firstly, recall the definitions for the set of 
critical and saddle points 
\begin{equation}
\begin{aligned}
	\mathcal{C} 
		&:= \left\{ y \in M | \grad F(y) = 0 \right\} \,, \\
	\mathcal{S} 
		&:= \left\{ y \in \mathcal{S} \, | \, 
			\lambda_{\max}( \nabla^2 F(y) ) > 0 \,, 
			\lambda_{\min}( \nabla^2 F(y) ) < 0 
			\right\} \,, 
\end{aligned}
\end{equation}
also recall that when $F$ is Morse both sets are finite. 

Using the construction from 
\cref{subsec:perturb_construction}, 
and denoting each constant $\delta, \wt{\delta}, \ell$ 
as a function of $y \in \mathcal{S}$, 
we can finally define the perturbation as 
\begin{equation}
\label{eq:perturb_potential_on_M}
	\wt{F}_\beta(x) 
	:= 
		F(x) + \sum_{y \in \mathcal{S}} 
			\xi( d_{ \delta(y), y }(x)^2 ) \,, 
\end{equation}
where $\xi$ is the smooth cutoff function 
constructed in \cref{lm:smooth_cutoff}. 

We will further introduce several additional constants 
\begin{equation}
\begin{aligned}
	\delta_{\min} 
		&:= \min_{ y \in \mathcal{S} } \delta(y) \,, \\
	\wt{\lambda}
		&:= \min_{ y \in \mathcal{C} \setminus \{x^*\} } 
			\sum_{i=1}^{nd} 
			\left[ - \lambda_i( \nabla^2 F(y) ) \right]_+ \,, 
\end{aligned}
\end{equation}
where $x^* \in \mathcal{C}$ is the unique global minimum of $F$, 
and $[x]_+ := \max(x, 0)$. 

Here we additionally observe the following estimate 
for all $y \in \mathcal{S}$ 
\begin{equation}
	\frac{1}{2} \wt{\lambda} 
	\leq 
		\wt{\delta}(y) 
	\leq 
		(2\ell(y) - nd) \delta(y) + \sum_{i=1}^{\ell(y)} |\lambda_i| 
	\leq 
		2 nd K_2 \,, 
\end{equation}
where we used the definition of \cref{eq:delta_tilde_defn}. 


\begin{lemma}
[Lyapunov Condition Near a Saddle Point]
\label{lm:lyapunov_near_saddle}
Suppose $F$ satisfies 
\cref{asm:app_c3,asm:app_morse,asm:app_unique_min}. 
Let $y \in \mathcal{S}$ be a non-degenerate saddle point. 
Then for all choices of $a,\beta > 0$ such that 
\begin{equation}
\begin{aligned}
	a^2 
	&\geq 
		\frac{8K_2^2}{\delta_{\min}^2} 
		[ (n+1) d+32 ] 
		\,, \\
	\beta 
	&\geq 
		C a^2 (nd)^4 
			\max( \delta_{\min}^{-1}, \delta_{\min}^{-7} ) 
			\max( \wt{\lambda}^{-1}, 1 )
			\max( K_2^{-1}, K_2^6 ) 
			\max( K_3^2, K_3^4 ) \,, 
\end{aligned}
\end{equation}
where $C > 0$ is a universal constant, 
we have the following Lyapunov condition 
\begin{equation}
	\frac{\Delta \wt{F}_\beta(x)}{2} 
	- \frac{\beta}{4} | \grad \wt{F}_\beta(x) |_g^2 
	\leq 
		\frac{-\wt{\lambda}}{8} 
		\,, \quad 
	\forall \, x \in M : d_{\delta(y),y}(x)^2 \leq \frac{a^2}{\beta} \,. 
\end{equation}
\end{lemma}



\begin{proof}

We start by observing that the choice of $\beta$ 
is simply a combination of the conditions of 
\cref{lm:perturb_laplacian_upper_bound,lm:perturb_grad_lower_bound}, 
but written in a way to reduce the complexity of the expression. 
More precisely, the original condition is 
\begin{equation}
\begin{aligned}
	\beta 
	\geq 
		a^2 \max \bigg( &
			\frac{4 d n^{1/2} }{\delta} \,, 
			\frac{ 2 n d K_2^{1/2} }{ 3 \delta^{3/2} } \,, 
			\frac{1}{2 K_2} \,, 
			\frac{ 2 n d K_2^{1/2} }{ 3 \delta^2 } \,, 
			\\ 
		& 
		\frac{ 16 K_2^2 }{ \delta^4 }
			\left[ 
				\frac{ 100 K_3^2 + 8710 (n d K_2)^2 }{ \delta^{3/2} }
				+ \frac{ 2\pi^2 (K_3 + 4\pi nd K_2) K_2^{1/2} }{ \delta }
				+ \frac{\pi K_2}{\delta^{1/2}} 
			\right]^{2} 
		\bigg) \,, 
\end{aligned}
\end{equation}
and we observe the fact that $n,d \geq 1$, 
but all other variables $\delta, K_2, K_3$ 
could be either greater than or smaller than $1$, 
so we need the both the largest and smallest power. 
We will also assume 
\begin{equation}
	\beta \geq a^2 \frac{ 8 n^{3/2} d^2 K_2 }{ \wt{\delta} \delta }
\end{equation}

Putting this together with the facts that 
$\delta(y) \geq \delta_{\min}$ 
and $\wt{\delta} \geq \frac{1}{2} \wt{\lambda}$, 
we get the $\beta$ condition 
in the lemma statement. 



\vspace{0.2cm}
\noindent
\textbf{Case 1. } 
$d_{\delta,y}(x)^2 \leq \frac{a^2}{4 \beta}$. 

We will directly compute the Lyapunov condition 
\begin{equation}
\begin{aligned}
	\frac{\Delta \wt{F}_\beta(x)}{2} 
		- \frac{\beta}{4} | \grad \wt{F}_\beta(x) |_g^2 
	&\leq 
		\frac{\Delta \wt{F}_\beta(x)}{2} 
		\\ 
	&= 
		\frac{1}{2} 
		\left[ \Delta F(x) 
			+ \xi'' | \grad d_{\delta,y}(x)^2 |_g 
			+ \xi' \Delta d_{\delta,y}(x)^2
		\right] \,, 
\end{aligned}
\end{equation}
and here we recall by construction 
\cref{lm:smooth_cutoff} 
we have that $\xi' = -1$ 
when $d_{\delta,y}(x)^2 \leq \frac{a^2}{4\beta}$, 
and therefore $\xi'' = 0$. 

We further recall \cref{lm:grad_laplacian_prod_approx} 
so that we can write 
\begin{equation}
\begin{aligned}
	\frac{1}{2} 
		\left[ \Delta F(x) 
			+ \xi'' | \grad d_{\delta,y}(x)^2 |_g 
			+ \xi' \Delta d_{\delta,y}(x)^2
		\right]
	&= 
		\frac{1}{2} 
			\sum_{i=1}^{nd} \lambda_i 
			- c_i \Delta \frac{1}{2} 
			\langle x, u_i \rangle^2 
			\\ 
	&\leq 
		\frac{1}{2} 
			\sum_{i=1}^{nd}
			\lambda_i - c_i 
			+ c_i 2 d \sqrt{n} |x|^2 
			\\ 
	&\leq 
		\frac{1}{2} 
			\sum_{i=1}^{nd}
			(\lambda_i - c_i)
		+ \frac{2 n^{3/2} d^2 K_2}{\delta} d_{\delta,y}(x)^2 \,, 
\end{aligned}
\end{equation}
where we used the fact that $c_i \leq K_2$ 
and the norm estimates from \cref{eq:delta_norm_est}. 

Here we will observe that 
\begin{equation}
	\sum_{i=1}^{nd} \lambda_i - c_i 
	= 
		\sum_{i=1}^\ell (\lambda_i - \delta) 
		+ \sum_{i = \ell+1}^{nd} \lambda_i - (\lambda_i - \delta) 
	= 
		\sum_{i=1}^\ell \lambda_i + (n-2\ell) \delta
	= 
		- \wt{\delta} \,, 
\end{equation}
where we recall the definition of $\wt{\delta}$ 
from \cref{eq:delta_tilde_defn}. 

At this point, we will also plug in the condition that 
$d_{\delta,y}(x)^2 \leq \frac{a^2}{4 \beta}$ to get 
\begin{equation}
	\frac{1}{2} 
			\sum_{i=1}^{nd}
			(\lambda_i - c_i)
		+ \frac{2 n^{3/2} d^2 K_2}{\delta} d_{\delta,y}(x)^2 
	\leq 
		\frac{ - \wt{\delta} }{2} 
		+ \frac{n^{3/2} d^2 K_2}{2 \delta} \frac{a^2}{\beta}
		\,, 
\end{equation}
and we can choose 
\begin{equation}
	\frac{a^2}{\beta} 
	\leq 
		\frac{ \wt{\delta} \delta }{ 8 n^{3/2} d^2 K_2 } \,, 
\end{equation}
to get the desired result of 
\begin{equation}
	\frac{ - \wt{\delta} }{2} 
		+ \frac{n^{3/2} d^2 K_2}{2 \delta} \frac{a^2}{\beta}
	\leq 
		\frac{ -\wt{\delta} }{4} 
	\leq 
		\frac{ -\wt{\lambda} }{8} \,. 
\end{equation}






\vspace{0.2cm}
\noindent
\textbf{Case 2. } 
$ d_{\delta,y}(x)^2 \in 
\left[ \frac{a^2}{4\beta}, \frac{a^2}{\beta} \right] $

For this section, 
we will use the estimates from 
\cref{lm:perturb_laplacian_upper_bound,lm:perturb_grad_lower_bound}
to write 
\begin{equation}
	\frac{\Delta \wt{F}_\beta(x)}{2} 
		- \frac{\beta}{4} | \grad \wt{F}_\beta(x) |_g^2 
	\leq 
		\frac{ K_2(d+32) }{2}
		- \frac{\beta}{4} \frac{ \delta^2 }{ 4 K_2 } \frac{a^2}{\beta} \,, 
\end{equation}
and we will use the choice of 
\begin{equation}
	a^2 
	\geq 
		\frac{8K_2^2}{\delta_{\min}^2} 
		[ (n+1) d+32 ] 
	\geq 
		\frac{K_2}{\delta^2} 
		[ 4 \wt{\delta} + 8K_2 (d+32) ] \,, 
\end{equation}
where we used the estimate $\wt{\delta} \leq 2 nd K_2$, 
which gives us the desired result 
\begin{equation}
	\frac{ K_2(d+32) }{2}
		- \frac{\beta}{4} \frac{ \delta^2 }{ 4 K_2 } \frac{a^2}{\beta} 
	\leq 
		\frac{ -\wt{\delta} }{4} 
	\leq 
		\frac{ -\wt{\lambda} }{8}
		\,. 
\end{equation}

\end{proof}




















\begin{lemma}
[Lyapunov Condition Near a Local Maximum]
\label{lm:lyapunov_near_local_max}
Suppose $F$ satisfies 
\cref{asm:app_c3,asm:app_morse,asm:app_unique_min}. 
Let $y \in \mathcal{C}$ be a local maximum, 
i.e. $\lambda_{\max}(\nabla^2 F(y)) < 0$. 
Then for all choices of $a,\beta > 0$ such that 
\begin{equation}
\begin{aligned}
	\frac{a^2}{\beta} 
	\leq 
		\frac{ 9 \wt{\lambda}^2 \delta_{\min} }{ 8 (K_3 nd )^2 } \,, 
\end{aligned}
\end{equation}
we have the following Lyapunov condition 
\begin{equation}
	\frac{\Delta F(x)}{2} 
		- \frac{\beta}{4} | \grad F(x) |_g^2 
	\leq 
		\frac{-\wt{\lambda}}{8} 
		\,, \quad 
	\forall \, x \in M : d_{\delta_{\min},y}(x)^2 
		\leq \frac{a^2}{\beta} \,. 
\end{equation}
\end{lemma}

\begin{proof}

We begin by using the fact that 
the Hessian is $K_3$-Lipschitz to write 
\begin{equation}
	\frac{\Delta F(x)}{2} 
		- \frac{\beta}{4} | \grad F(x) |_g^2 
	\leq 
		\frac{1}{2} \Delta F(y) 
		+ \frac{1}{2} | \Delta F(x) - \Delta F(y) | 
	\leq 
		\frac{1}{2} \sum_{i=1}^{nd} \lambda_i 
			+ \frac{1}{2} K_3 nd |x| \,. 
\end{equation}

Using the norm estimates in \cref{eq:delta_norm_est} 
with $\delta_{\min}$, 
and the definition of $\wt{\lambda}$, 
we can write 
\begin{equation}
	\frac{1}{2} \sum_{i=1}^{nd} \lambda_i 
		+ \frac{1}{2} K_3 nd |x| 
	\leq 
		- \frac{\wt{\lambda}}{2} 
		+ \frac{K_3 nd}{\sqrt{2 \delta_{\min}}} d_{\delta_{\min},y}(x) 
	\leq 
		- \frac{\wt{\lambda}}{2} 
		+ \frac{K_3 nd}{\sqrt{2 \delta_{\min}}} \frac{a}{ \sqrt{\beta} } \,. 
\end{equation}

Finally, by choosing 
\begin{equation}
	\frac{a^2}{\beta} 
	\leq 
		\frac{ 9 \wt{\lambda}^2 \delta_{\min} }{ 8 (K_3 nd )^2 } \,, 
\end{equation}
we get the desired result of 
\begin{equation}
	- \frac{\wt{\lambda}}{2} 
		+ \frac{K_3 nd}{\sqrt{2 \delta_{\min}}} \frac{a}{ \sqrt{\beta} }
	\leq 
		\frac{ -\wt{\lambda} }{8} \,. 
\end{equation}

\end{proof}


















\begin{lemma}
[Morse Gradient Estimate]
\label{lm:morse_grad_est}
Suppose $F$ satisfies 
\cref{asm:app_c3,asm:app_morse,asm:app_unique_min}. 
Let $\mathcal{C}$ be the set of critical points of $F$. 
Then there exists a constant $C_F > 0$ such that 
\begin{equation}
	| \grad F(x) |_g \geq C_F \, d(x, \mathcal{C}) \,, 
\end{equation}
where $d(x, \mathcal{C})$ denotes 
the smallest geodesic distance between $x$ 
and a critical point $y \in \mathcal{C}$. 

In particular, we can write the constant explicitly as 
\begin{equation}
	C_F := \min \left( \frac{ \lambda_* }{2} \,, 
			\inf_{ x : d(x, \mathcal{C}) > \frac{\lambda_*}{2 K_3} } 
			\frac{ |\grad F|_g }{ d(x, \mathcal{C}) }
			\right) \,, 
\end{equation}
where we define 
\begin{equation}
	\lambda_* 
	:= 
		\min_{y \in \mathcal{C}} \min_{i \in [nd]} 
		| \lambda_i ( \nabla^2 F(y) ) | 
		\,. 
\end{equation}

\end{lemma}

\begin{proof}

First, observe that since 
\begin{equation}
	\inf_{ x : d(x, \mathcal{C}) > \frac{\lambda_*}{2 K_3} } 
		\frac{ |\grad F|_g }{ d(x, \mathcal{C}) } 
	> 0 \,, 
\end{equation}
due to the fact that $M$ is compact and $F$ is Morse, 
then it is sufficient to consider only 
$x \in M$ such that 
$d(x,\mathcal{C}) \leq \frac{ \lambda_* }{ 2K_3 }$. 

Let $y \in \mathcal{C}$ be a critical such that 
$d(x,y) = d(x, \mathcal{C})$, 
and let $\gamma(t)$ be a geodesic such that 
$\gamma(0) = y, \gamma(1) = x$. 
Let $D_t$ be the covariant time derivative along $\gamma(t)$, 
then we have that 
\begin{equation}
	| D_t \lambda_i ( \nabla^2 F(\gamma(t)) ) | 
	\leq 
		| D_t \nabla^2 F(\gamma(t)) |_g 
	= 
		| \nabla^3 F( \gamma(t) )^\sharp[ \dot{\gamma}(t) ] |_g 
	\leq 
		K_3 | \dot{\gamma}(t) |_g 
	= 
		K_3 d(x,y)
		\,, 
\end{equation}
where we used the fact that $\lambda_i$ is $1$-Lipschitz, 
and $\sharp$ denotes the musical isomorphism of raising an index 
\citep{lee2019riemann}. 
This further implies 
\begin{equation}
	| \lambda_i ( \nabla^2 F(x) ) 
		- \lambda_i ( \nabla^2 F(y) ) | 
	\leq 
		K_3 d(x,y)
	\leq 
		\frac{\lambda_*}{ 2 } \,. 
\end{equation}

Now we will repeat the same procedure for the gradient 
\begin{equation}
	| D_t \grad F( \gamma(t) ) |_g 
	= 
		| \nabla^2 F( \gamma(t) )^\sharp [ \dot{\gamma}(t) ] |_g 
	\geq 
		\min_{i \in [nd]} | \lambda_i ( \nabla^2 F(x) ) | \, 
		|\dot{\gamma}(t)| 
	\geq 
		\frac{\lambda_*}{2} d(x,y) \,. 
\end{equation}

At this point, we can recover the desired $C_F > 0$ 
by taking the minimum of the two constants. 

\end{proof}














\begin{lemma}
[Lyapunov Condition Away From Critical Points]
\label{lm:lyapunov_away_from_crit}
Suppose $F$ satisfies 
\cref{asm:app_c3,asm:app_morse,asm:app_unique_min}. 
Let $\mathcal{C}$ be the set of critical points. 
Then for all choices of $a,\beta > 0$ such that 
\begin{equation}
\begin{aligned}
	a^2 
	&\geq 
		\frac{ 2K_2^2 nd }{ C_F^2 } 
		\,, 
\end{aligned}
\end{equation}
we have the following Lyapunov condition 
\begin{equation}
	\frac{\Delta F(x)}{2} 
	- \frac{\beta}{4} | \grad F(x) |_g^2 
	\leq 
		\frac{-\wt{\lambda}}{8} 
		\,, \quad 
	\forall \, x \in M : d(x, \mathcal{C})^2 
		\geq \frac{2a^2}{K_2 \beta} \,. 
\end{equation}
\end{lemma}


\begin{proof}

We begin by directly computing the Lyapunov condition 
using \cref{lm:morse_grad_est}
\begin{equation}
	\frac{\Delta F(x)}{2} 
	- \frac{\beta}{4} | \grad F(x) |_g^2 
	\leq 
		\frac{ K_2 nd }{ 2 } 
		- \frac{\beta}{4} C_F^2 d(x, \mathcal{C})^2 \,, 
\end{equation}
and using the choice 
$d(x, \mathcal{C})^2 \geq \frac{2a^2}{K_2 \beta}$, 
we can get 
\begin{equation}
	\frac{ K_2 nd }{ 2 } 
		- \frac{\beta}{4} C_F^2 d(x, \mathcal{C})^2
	\leq 
		\frac{ K_2 nd }{ 2 } 
		- \frac{\beta}{4} C_F^2 \frac{2a^2}{K_2 \beta} \,. 
\end{equation}

Now we will use the choice that 
\begin{equation}
	a^2 
	\geq 
		\frac{ 2K_2^2 nd }{ C_F^2 } 
	\geq 
		\left[ \frac{\wt{\lambda}}{8} + \frac{K_2 nd}{ 2 } 
		\right] 
		\frac{2K_2}{ C_F^2 } \,, 
\end{equation}
which gives us the desired result of 
\begin{equation}
	\frac{ K_2 nd }{ 2 } 
		- \frac{\beta}{4} C_F^2 \frac{2a^2}{K_2 \beta} 
	\leq 
		\frac{ -\wt{\lambda} }{ 8 } \,. 
\end{equation}

\end{proof}










\begin{proposition}
[Lyapunov Condition on the Entire Manifold]
\label{prop:lyapunov_entire_manifold}
Suppose $F$ satisfies 
\cref{asm:app_c3,asm:app_morse,asm:app_unique_min}. 
Then for all choices of $a,\beta > 0$ such that 
\begin{equation}
\begin{aligned}
	a^2 
	&\geq 
		\max\left( 
			\frac{8 K_2^2}{\delta_{\min}^2} 
				[ (n+1)d + 32 ] \,, 
			\frac{2 K_2^2 nd}{ C_F^2 } 
			\right)
			\,, \\
	\beta 
	&\geq
		C a^2 (nd)^4 
			\max( \delta_{\min}^{-1}, \delta_{\min}^{-7} ) 
			\max( \wt{\lambda}^{-2}, 1 )
			\max( K_2^{-1}, K_2^6 ) 
			\max( K_3^2, K_3^4 ) \,, 
\end{aligned}
\end{equation}
where $C > 0$ is a universal constant, 
we have the following Lyapunov condition 
\begin{equation}
	\frac{\Delta \wt{F}_\beta(x)}{2} 
	- \frac{\beta}{4} | \grad \wt{F}_\beta(x) |_g^2 
	\leq 
		\frac{-\wt{\lambda}}{8} 
		+ 
		K_2 nd \mathds{1}_U(x) \,, 
\end{equation}
where $U := \{ x \in M | d(x,x^*)^2 \leq \frac{2a^2}{K_3 \beta} \}$. 

\end{proposition}

\begin{proof}

We start by consider $x \in M$ such that 
$d(x,x^*) > \frac{2a^2}{K_3 \beta}$, 
i.e. $x \not in U$.  
Here we observe that the condition on $a^2$ 
is simply combing the results of 
\cref{lm:lyapunov_near_saddle,lm:lyapunov_away_from_crit}. 
And the condition on $\beta$ is only modified 
from \cref{lm:lyapunov_near_saddle} 
to include $\beta \geq O( \wt{\lambda}^{-2} )$ 
from \cref{lm:lyapunov_near_local_max}. 
Also observe that for all $\delta > 0$
\begin{equation}
	d(x,y)^2 \geq \frac{2 a^2}{ K_2 \beta } 
	\implies 
	d_{\delta,y}(x)^2 \geq \frac{a^2}{\beta} \,, 
\end{equation}
which means the Lyapunov condition is satisfied 
using \cref{lm:lyapunov_near_saddle,lm:lyapunov_near_local_max,lm:lyapunov_away_from_crit} together. 

Finally, we consider when $x \in U$, 
and the desired result follows from 
\begin{equation}
	\frac{\Delta \wt{F}_\beta(x)}{2} 
		- \frac{\beta}{4} | \grad \wt{F}_\beta(x) |_g^2 
	\leq 
		\frac{ K_2 nd }{2} 
	= 
		\frac{ -\wt{\lambda} }{8} 
		+ \left[ 
			\frac{ \wt{\lambda} }{8} 
			+ \frac{ K_2 nd }{2} 
			\right] 
	\leq 
		\frac{ -\wt{\lambda} }{8} 
		+ K_2 nd \mathds{1}_U(x) \,, 
\end{equation}
where we used the upper bound $\wt{\lambda} \leq K_2 nd$. 

\end{proof}
















\subsection{Lyapunov to Poincar\'{e} and LSI}

Before we start this subsection, 
we refer to \cref{subsec:app_lyapunov} 
for existing results on Lyapunov conditions, 
which we lightly adapted to our setting. 





\begin{proposition}
[Poincar\'{e} Inequality]
\label{prop:lyapunov_poincare}
Suppose $F$ satisfies 
\cref{asm:app_c3,asm:app_morse,asm:app_unique_min}. 
Then for all choices of $a,\beta > 0$ such that 
\begin{equation}
\begin{aligned}
	a^2 
	&\geq 
		\max\left( 
			\frac{8 K_2^2}{\delta_{\min}^2} 
				[ (n+1)d + 32 ] \,, 
			\frac{2 K_2^2 nd}{ C_F^2 } 
			\right)
			\,, \\
	\beta 
	&\geq
		C a^2 (nd)^4 
			\max( \delta_{\min}^{-1}, \delta_{\min}^{-7} ) 
			\max( \wt{\lambda}^{-2}, 1 )
			\max( \lambda_{\min}^{-2}, 1 )
			\max( K_2^{-1}, K_2^6 ) 
			\max( K_3^2, K_3^4 ) \,, 
\end{aligned}
\end{equation}
where $C > 0$ is a universal constant, 
we have that the Markov triple $(M,\wt{\nu},\Gamma)$ with 
$\wt{\nu}_\beta \propto \exp( -\beta \wt{F}_\beta )$ 
satisfies a Poincar\'{e} inequality with constant 
\begin{equation}
	\wt{\kappa} 
	= 
		\frac{ \wt{\lambda} / 8 }{ 
			1 + {2 K_2 nd }/{\lambda_{\min} } } \,, 
\end{equation}
where we define $\lambda_{\min} := \lambda_{\min}( \nabla^2 F(x^*) )$. 

Furthermore, the unperturbed Markov triple 
$(M,\nu,\Gamma)$ with 
$\nu \propto \exp( -\beta F )$ 
satisfies a Poincar\'{e} inequality with constant 
\begin{equation}
	\kappa
	= 
		\frac{ \wt{\lambda} / 8 }{ 
			1 + {2 K_2 nd }/{\lambda_{\min} } } 
		e^{-a^2} \,. 
\end{equation}


\end{proposition}

\begin{proof}

We start by observing that the condition on $\beta$ 
is further modified from \cref{prop:lyapunov_entire_manifold} 
to include 
\begin{equation}
	\beta \geq a^2 \frac{ 8 K_3 }{ \lambda_{\min}^2 } \,. 
\end{equation}

We will next derive a Poincar\'{e} inequality on the set 
$U := \{ x \in M | d(x, x^*)^2 \leq \frac{2a^2}{K_3 \beta} \}$. 
Using the same idea as \cref{lm:morse_grad_est}, 
we will observe that for $x \in U$
\begin{equation}
	\min_{i \in [nd]} \lambda_i ( \nabla^2 F(x) ) 
	\geq 
		\lambda_{\min} 
		- K_3 d(x,x^*) 
	\geq 
		\frac{ \lambda_{\min} }{2} \,, 
\end{equation}
where we used the choice of 
$\beta \geq a^2 \frac{ \lambda_{\min}^2 }{ 8 K_3 }$ 
to get 
$d(x, x^*)^2 \leq \frac{2a^2}{K_3 \beta} 
\leq \frac{\lambda_{\min}}{2K_3}$. 

It follows from the curvature dimension condition 
\citep[Proposition 4.8.1]{bakry2013analysis} 
that $\wt{\nu}_\beta$ (and $\nu$) satisfies 
a Poincar\'{e} inequality on $U$ with constant 
$\kappa_U = \frac{1}{2} \lambda_{\min}$. 

Then we will observe that the Lyapunov condition 
in \cref{prop:lyapunov_entire_manifold} can also be 
stated as follows 
\begin{equation}
	\frac{L W}{ W } 
	= \frac{1}{2} \Delta \wt{F}_\beta(x) 
		- \frac{\beta}{4} |\grad \wt{F}_\beta(x)|_g^2 
	\leq \theta + b \mathds{1}_U \,, 
\end{equation}
where we choose the Lyapunov function 
$W := \exp( -\beta \wt{F}_\beta )$. 


Next, we observe that $F \geq 0$ implies 
this condition readily translates 
to the Lyapunov condition for Poincar\'{e} inequality 
\cref{thm:lyapunov_poincare_bakry}, 
with $\theta = \wt{\lambda} / 8, b = K_2 nd, 
\kappa_U = \lambda_{\min}/2$ 
to get that $(M, \wt{\nu}_\beta), \Gamma$ 
satisfies a Poincar\'{e} inequality with constant 
\begin{equation}
	\wt{\kappa} 
	= \frac{\theta}{ 1 + b / \kappa_U } 
	= \frac{ \wt{\lambda} / 8 }{ 1 + 2 K_2 nd / \lambda_{\min} } 
	\,. 
\end{equation} 

Finally, we will recall the Holley--Stroock perturbation 
\citep[Proposition 4.2.7]{bakry2013analysis}, 
which states that $(M,\nu,\Gamma)$ satisfies 
a Poincar\'{e} inequality with constant 
\begin{equation}
	\wt{\kappa} \exp( -\beta \Osc(\wt{F}_\beta - F)) 
	\geq 
		\frac{ \wt{\lambda} / 8 }{ 1 + 2 K_2 nd / \lambda_{\min} } 
		\exp( -a^2 ) 
	=:
		\kappa \,, 
\end{equation}
where we used the fact that 
$\Osc(\wt{F}_\beta - F) \leq \frac{a^2}{\beta}$ 
from \cref{lm:smooth_cutoff}. 

\end{proof}
























\begin{lemma}
[Second Moment Bound from Lyapunov Condition]
\label{lm:lyapunov_second_moment_bound}
Let $\nu = \frac{1}{Z} \exp( -\beta F)$ 
such that there exists a Lyapunov function 
$W:M \to [1,\infty)$ satisfying 
\begin{equation}
	\frac{LW}{W} \leq - \theta + b \mathds{1}_{B_R(x_0)} \,, 
\end{equation}
for some constants $\theta, b > 0$, 
then we have that 
\begin{equation}
	\int_M d(x,x_0)^2 \, d\nu 
	\leq 
		\frac{1 + b \beta R^2}{ c \beta } \,. 
\end{equation}
\end{lemma}

\begin{proof}

Using an intermediate step of 
\cref{thm:lyapunov_poincare_bakry}, 
we have that for all $h \in C^1(M) \cap L^2(\nu)$ 
 
\begin{equation}
	\int_M h^2 \, d\nu 
	\leq 
		\frac{1}{c\beta} \int_M |\grad h|_g^2 \, d\nu 
		+ \frac{b\beta}{c\beta} 
			\int_{B_R(x_0)} h^2 \, d\nu \,. 
\end{equation}

At this point, we can choose $h(x) = d(x,x_0)$, 
and observe that 
\begin{equation}
	| \grad h |_g 
	= 
		\left| \frac{ -\log_x(x_0) }{ |\log_x (x_0)|_g }
		\right|_g 
	= 
		1 \,. 
\end{equation}

The desired follows through direct computation 
\begin{equation}
	\frac{1}{c\beta} \int_M |\grad h|_g^2 \, d\nu 
		+ \frac{b\beta}{c\beta} 
			\int_{B_R(x_0)} h^2 \, d\nu 
	\leq 
		\frac{1}{c\beta} + \frac{b\beta R^2}{c\beta} \,. 
\end{equation}

\end{proof}





We will now restate the main result from 
\cref{thm:lyapunov_log_sobolev}. 

\begin{theorem}
[Logarithmic Sobolev Inequality]
Suppose $F$ satisfies 
\cref{asm:app_c3,asm:app_morse,asm:app_unique_min}. 
Then for all choices of $a>0,\beta \geq 1$ such that 
\begin{equation}
\begin{aligned}
	a^2 
	&\geq 
		\max\left( 
			\frac{8 K_2^2}{\delta_{\min}^2} 
				[ (n+1)d + 32 ] \,, 
			\frac{2 K_2^2 nd}{ C_F^2 } 
			\right)
			\,, \\
	\beta 
	&\geq
		C a^2 (nd)^4 
			\max( \delta_{\min}^{-1}, \delta_{\min}^{-7} ) 
			\max( \wt{\lambda}^{-2}, 1 )
			\max( \lambda_{\min}^{-2}, 1 )
			\max( K_2^{-1}, K_2^6 ) 
			\max( K_3^2, K_3^4 ) \,, 
\end{aligned}
\end{equation}
where $C > 0$ is a universal constant, 
there exists a perturbation $\wt{F}_\beta \in C^3(M)$ 
parameterized by $a, \beta$ such that 
\begin{equation}
	\| \wt{F}_\beta - F \|_\infty \leq \frac{a^2}{\beta} \,, 
\end{equation}
and we have that the Markov triple $(M,\wt{\nu},\Gamma)$ with 
$\wt{\nu}_\beta(dx) = \frac{1}{\wt{Z}} \exp( -\beta \wt{F}_\beta )\,dx$ 
satisfies $\LSI(\wt{\alpha})$ where 
\begin{equation}
	\frac{1}{\wt{\alpha}} 
	= 
		\left[ 
			\sqrt{ 
				\frac{2(1 + \frac{2a^2b}{K_3})}{c \wt{\kappa}} 
			} 
			+ \frac{2 K_2 (1 + \frac{2a^2b}{K_3})}{c \wt{\kappa}} 
			+ \frac{4}{c \wt{\kappa}} 
		\right] 
		+ 
		\beta \left[ 
			\sqrt{ 
				\frac{2}{c} \left( 
				1 + \frac{b}{\wt{\kappa}} 
				\right) 
				}
			+ 
				\frac{K_2}{c} 
				\left( 1 + \frac{2b}{\wt{\kappa}} 
				\right) 
		\right] \,. 
\end{equation}

Furthermore, the unperturbed Markov triple 
$(M,\nu,\Gamma)$ with 
$\nu \propto \exp( -\beta F )$ 
satisfies $\LSI(\alpha)$ with constant 
\begin{equation}
	\alpha 
	= 
		\wt{\alpha} 
		e^{-a^2} 
	= 
		\Omega\left( \frac{1}{1+\beta} \right) \,, 
\end{equation}
where we use $\Omega(\cdot)$ to show only dependence on $\beta$. 

\end{theorem}

\begin{proof}

We start by showing that $\wt{\nu}_\beta$ 
satisfies the Lyapunov condition of 
\cref{prop:lyapunov_log_sobolev_cattiaux}. 
This follow easily by observing that 
for all $x_0 \in M$ we have that 
\begin{equation}
	d(x,x_0)^2 
	\leq 
		n \pi \,, 
\end{equation}
then we have that \cref{prop:lyapunov_entire_manifold} implies 
\begin{equation}
	\frac{LW}{W} 
	\leq 
		- \frac{\wt{\lambda}}{8 n\pi} d(x,x_0)^2 
		+ K_2 nd \,. 
\end{equation}

Next we further observe that since $\grad F$ 
is $K_2$-Lipschitz, 
and that $\Ric_g \geq 0$, 
we also satisfies the curvature condition 
\begin{equation}
	\nabla^2 F + \frac{1}{\beta} \Ric_g 
	\geq - K_2 g \,. 
\end{equation}

Finally, recalling that $\wt{\nu}_\beta$ also satisfies 
a Poincar\'{e} inequality from 
\cref{prop:lyapunov_poincare}, 
now \cref{prop:lyapunov_log_sobolev_cattiaux} 
implies $\wt{\nu}_\beta$ satisfies a logarithmic Sobolev inequality 
with constant 
\begin{equation}
	\frac{1}{\wt{\alpha} \, \beta} 
	= 
		\sqrt{ \frac{2}{c\beta} \left( 
		1 + \frac{b \beta + \nu(\phi)}{\beta \wt{\kappa}} 
		\right) } 
		+ 
		\frac{K_2}{c} 
		+ \frac{2}{c \beta \beta \wt{\kappa}} \left( 
			\beta K_2 ( b \beta + \nu(\phi)) + 2
		\right) \,, 
\end{equation}
where $c = \frac{\wt{\lambda}}{8\pi n}$, 
$b = K_2 nd$, 
and $\phi = c\,\beta\,d(x,x_0)^2$. 

Now we can also use the second moment bound from 
\cref{lm:lyapunov_second_moment_bound} 
with the condition $R^2 \leq \frac{2a^2}{K_3\beta}$ 
from \cref{prop:lyapunov_entire_manifold}, 
which lets us bound 
\begin{equation}
	\nu(\phi) 
	\leq 
		1 + b \beta \frac{2a^2}{K_3 \beta} 
	= 
		1 + \frac{2a^2 b}{K_3} \,. 
\end{equation}

Now we can simplify the logarithmic Sobolev constant as 
\begin{equation}
	\frac{1}{\wt{\alpha} \, \beta} 
	\leq 
		\sqrt{ 
			\frac{1}{\beta} \frac{2}{c} \left( 
			1 + \frac{b}{\wt{\kappa}} 
			\right) 
			+ \frac{1}{\beta^2} 
			\frac{2(1 + \frac{2a^2b}{K_3})}{c \wt{\kappa}} 
			} 
		+ 
			\frac{K_2}{c} \left( 1 + \frac{2b}{\wt{\kappa}} 
			\right)
		+ 
			\frac{1}{\beta} 
			\frac{2 K_2 (1 + \frac{2a^2b}{K_3})}{c \wt{\kappa}} 
		+ 
			\frac{1}{\beta^2} 
			\frac{4}{ c \wt{\kappa} } \,. 
\end{equation}

Using the inequality $\sqrt{a+b} \leq \sqrt{a} + \sqrt{b}$ 
for $a,b \geq 0$, 
we can further write 
\begin{equation}
	\frac{1}{\wt{\alpha} \, \beta} 
	\leq 
		\frac{K_2}{c} \left( 1 + \frac{2b}{\wt{\kappa}} 
			\right)
		+
			\sqrt{ 
				\frac{1}{\beta} \frac{2}{c} \left( 
				1 + \frac{b}{\wt{\kappa}} 
				\right) 
			}
		+ \frac{1}{\beta} 
			\left[ 
			\sqrt{ 
				\frac{2(1 + \frac{2a^2b}{K_3})}{c \wt{\kappa}} 
			} 
			+ \frac{2 K_2 (1 + \frac{2a^2b}{K_3})}{c \wt{\kappa}} 
			\right] 
		+ 
			\frac{1}{\beta^2} 
			\frac{4}{ c \wt{\kappa} } \,. 	
\end{equation}

Choosing $\beta \geq 1$, we can further simplify as 
\begin{equation}
	\frac{1}{\wt{\alpha}} 
	\leq 
		\left[ 
			\sqrt{ 
				\frac{2(1 + \frac{2a^2b}{K_3})}{c \wt{\kappa}} 
			} 
			+ \frac{2 K_2 (1 + \frac{2a^2b}{K_3})}{c \wt{\kappa}} 
			+ \frac{4}{c \wt{\kappa}} 
		\right] 
		+ 
		\beta \left[ 
			\sqrt{ 
				\frac{2}{c} \left( 
				1 + \frac{b}{\wt{\kappa}} 
				\right) 
				}
			+ 
				\frac{K_2}{c} 
				\left( 1 + \frac{2b}{\wt{\kappa}} 
				\right) 
		\right] \,. 
\end{equation}

Finally, since $F$ is a perturbation of $\wt{F}_\beta$, 
we have that by Holley--Stroock perturbation 
\citep[Proposition 5.1.6]{bakry2013analysis}, 
$\nu$ satisfies a logarithmic Sobolev inequality with constant 
\begin{equation}
	\alpha = \wt{\alpha} e^{-a^2} \,. 
\end{equation}

\end{proof}










==> temp_calc.tex <==

\section{Calculations}

\begin{equation}
d \begin{bmatrix}
	X_t \\ Y_t 
\end{bmatrix}
= 
	\left( \begin{bmatrix}
		0 & \lambda \\ 
		\lambda/2 & 0 
		\end{bmatrix} 
		\begin{bmatrix}
			X_t \\ Y_t 
		\end{bmatrix}
		+ 
		\begin{bmatrix}
			2/\beta \\ 0 
		\end{bmatrix}
	\right) \, dt
	+ 
	\frac{2}{\sqrt{\beta}} 
	\begin{bmatrix}
		\sqrt{X_t + Y_t} + \sqrt{X_t - Y_t} & 
		- \sqrt{X_t + Y_t} + \sqrt{X_t - Y_t} \\ 
		- \sqrt{X_t + Y_t} + \sqrt{X_t - Y_t} & 
		\sqrt{X_t + Y_t} + \sqrt{X_t - Y_t} 
	\end{bmatrix} \, 
	dB_t \,. 
\end{equation}


